Knowledge Enhanced Neural Networks for relational domains

In the recent past, there has been a growing interest in Neural-Symbolic Integration frameworks, i.e., hybrid systems that integrate connectionist and symbolic approaches to obtain the best of both worlds. In this work we focus on a specific method, KENN (Knowledge Enhanced Neural Networks), a Neural-Symbolic architecture that injects prior logical knowledge into a neural network by adding on its top a residual layer that modifies the initial predictions accordingly to the knowledge. Among the advantages of this strategy, there is the inclusion of clause weights, learnable parameters that represent the strength of the clauses, meaning that the model can learn the impact of each rule on the final predictions. As a special case, if the training data contradicts a constraint, KENN learns to ignore it, making the system robust to the presence of wrong knowledge. In this paper, we propose an extension of KENN for relational data. One of the main advantages of KENN resides in its scalability, thanks to a flexible treatment of dependencies between the rules obtained by stacking multiple logical layers. We show experimentally the efficacy of this strategy. The results show that KENN is capable of increasing the performances of the underlying neural network, obtaining better or comparable accuracies in respect to other two related methods that combine learning with logic, requiring significantly less time for learning.

==> Relational KENN/architecture.tex <==
\section{\kenn\ architecture}
\label{sec:architecture}
% This chapter is divided into two main sections: in the first one, it is defined a simple architecture for \kenn\ for multi-label classification tasks; in the second one we will introduce how to extend it for relational data.

% \section{Architecture}
% \label{sec:architecture}
As explained in Section~\ref{sec:kenn}, the core component of \kenn\
is in the \boost . In \kenn\ the \boost\ for a certain clause $c$ is
implemented by an architecture called \emph{Clause Enhancer} (CE), which is a
module instantiated that computes $\delta_c$ according to Equation~\eqref{eq:deltac}. 
Figure~\ref{fig:CE} shows the details of the architecture of the CE. 

% \subsection{Clause Enhancer}

\begin{figure}[H]
  \centering
	\input{tikz/CE}
	\caption{Clause Enhancer for $A \lor \lnot B$, where $A$ and $B$ are grounded atoms}
	\label{fig:CE}
\end{figure}

The CE receives as input a vector containing the preactivations generated by the base NN and it selects the right literals, returning $\bz_c$, the preactivations of the literals of clause $c$.
% the literals occurring in $c$ obtaining $\bz_c$, the preactivations of the literals of clause $c$. 
Then, Equation \ref{eq:delta_wc_s} of $\delta_s^w$ is applied. 
% Intuitively, the idea is that, in order to satisfy a clause, at least one of its literal must be true. The softmax function act as a selector for the most promising true literal, that is the one with highest supporting evidences (biggest preactivation).} 
The term $w_c$ is a positive weight associated to clause $c$ that represents the strength of $c$: the higher the $w_c$, the bigger the contribution of the clause in the final predictions. As opposed to methods based on the regularization of the Loss, $w_c$ is not a hyper parameter. On the contrary, it is a parameter of the model that is learned during training. This means that \kenn\ can discover the importance of each clause based on the data. As a special case of this behavior, it is possible for \kenn\ to learn to ignore clauses by setting $w_c$ to zero, making clause $c$ irrelevant for the final predictions.

The final step of the CE is a post elaboration that projects the proposed changes on the literals into changes to be applied on the atoms according to equation \ref{eq:deltac}.
% This operation corresponds to the Equation~\ref{eq:phip}.
%  for calculating $\delta_c$.

% \subsection{Knowledge Enhancer}

The outputs of the CEs are combined inside the \emph{Knowledge Enhancer} (KE), which is the final layer of \kenn\ model. Figure~\ref{fig:KE} shows the architecture of KE, which calculates the final interpretation as in Equation~\ref{eq:final_intepretation}.
%  Notice that a CE is instantiated for each grounded clause $c \in \G(\clauses, \C)$.

\begin{figure}[H]
	\centering
	\input{tikz/KE}
	\caption{Knowledge Enhancer architecture. It implements Equation~\ref{eq:final_intepretation} by summing the deltas values of each clause enhancer (one per grounded clause) with the initial preactivations $\bz$ and applying the logistic function }
	\label{fig:KE}
\end{figure}


% \subsection{Working with batches of data}
% In the architecture defined so far, since all the grounded atoms are inside the vector $\bz$, there are multiple instantiation of the same CE for each clause $c \in \clauses$, one for each grounding of $c$. For instance, in Figure~\ref{fig:KE_matrix}(a), the CE for clause $c: \lnot S(x) \lor C(x)$ is instantiated two times, one for object $a$, another for object $b$. 

% In many scenarios we want to use batches of data, which would require to modify the structure of the model graph for each batch, in particular after each training step, since the groundings are constantly changing and for each grounding a different CE is instantiated. Notice that, even if the CEs are different, the internal operations are the same and the only change is the provided input. For these reasons, we want to instantiate a single CE for each clause $c$ which works in a single batch containing all possible groundings of $c$.

% If the groundings involve a single object, a simple solution is to define $\bz$ as a matrix instead as a vector, where columns represent predicates and rows individuals. More in details, $\bz$ is now defined as a matrix such that the element $z_{ij}$ contains the preactivation of $P_j(o_i)$, with $P_j$ the $j^{th}$ predicate and $o_i$ the $i^{th}$ object. 
% Notice that this kind of representation is common when working with neural networks since the columns (predicates) correspond to the labels and the rows (groundings) to the samples. 

% Figure~\ref{fig:KE_matrix}(b) shows the overall idea. The CE is defined as before, but now it takes as input a matrix and it acts on each row separately. This can be done only if the same atom does not appear in multiple rows, since the changes are applied independently to each row and are not aggregated together. This property always holds with clauses that
% % have only unary predicates and 
% involve a single variable.
% % : we call this type of clauses \emph{unary}. In contrast, a clause that contains two variables is referred as a \emph{binary} clause. We define $\clauses_U$ as the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge can be described as $\clauses = \clauses_U \cup \clauses_B$.
% % For simplicity, in this thesis we don't take into account clauses with higher ariety. However, the proposed approach can be used with predicates and clauses with any number of variables.

% % As mentioned above, when dealing with unary clauses the approach of Fig~\ref{fig:KE_matrix}(b) can be used. 

% When a clause contain multiple variables, the same ground atom may occour in multiple groundings of the clause. 
% For instance, consider the clause 
% $$c: \lnot Smoke(x) \lor \lnot Friends(x,y) \lor Smoke(y)$$
% The two groundings $c[x/Alice,y/Bob]$ and $c[x/Bob,y/Carl]$ share a common grounded atom: $Smoke(Bob)$. For this reason, using a unique CE for $c$ is problematic since the values returned by the same CE are not aggregated, and we would end up with multiple changes proposed for the same atom.

% In the next sections, we will present the architecture of \kenn\ that can be used to instantiate a single CE even in relational domains, i.e. when dealing with predicates with arity greater than one.



% \begin{figure}[H]
% 	\centering
% 	\input{tikz/KE_matrix}
% 	\caption{KE applied on a Prior Knowledge consisting of a single clause $c$: $\lnot S(x) \lor C(x)$ applied on a domain of two objects ($a$ and $b$): (a) using a vector with all the grounded atoms, each grounding of $c$ is managed by a different CE.  Notice that the changes proposed by the first CE are zero for $C(b)$ and $S(b)$ while the second CE returns the value zero for the other two atoms: the two grounded clauses are independent; (b) using a matrix with a row for each grounding: all the grounding of $c$ are managed by the same CE, which operates in parallel on each row of the matrix. This is more convenient when dealing with mini-batches and results in a more efficient implementation.}
% 	\label{fig:KE_matrix}
% \end{figure}


% \subsection{KE for relational data}
% %\subsubsection{Unary and binary clauses}
% %\label{sec:SRL_representation}

% Maintaining a single vector with all the grounded atoms as in Section~\ref{sec:architecture} could lead to an inefficient implementation since it forces to create multiple CEs for each clause. This means that it requires to reset the computational graph every time new data is provided. On the other hand, in the approach of Fig.~\ref{fig:KE_matrix}(b), for each clause only a CE is instantiated and it can work in parallel on all the groundings of the clause. This has two advantages: it simplifies the usage of batches during training, and CEs' internal calculations are implemented as matrix operations, which are particularly efficient when working with a GPU. 

% However, such an approach can be applied with clauses that involve a single variable: we call this type of clauses \emph{unary}. In contrast, a clause that contains two variables is referred as a \emph{binary} clause. For simplicity, we don't take into account clauses with higher arity. Notice however that the proposed approach can be used with predicates and clauses with any number of variables.

% % We define $\clauses_U$ as the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge can be described as $\clauses = \clauses_U \cup \clauses_B$.
% % For simplicity, in this thesis we don't take into account clauses with higher ariety. However, the proposed approach can be used with predicates and clauses with any number of variables.

% % As mentioned above, when dealing with unary clauses the approach of Fig~\ref{fig:KE_matrix}(b) can be used. 


% % We introduce a classification for clauses based on the number of variables they contains: a clause is unary if it contains only one free variable, binary if it contains two variables. 

% Let $\clauses_U$ be the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge is now defined as $\clauses = \clauses_U \cup \clauses_B$.

% The idea now is to apply the KE to these two sets separately: Equation~\ref{eq:final_intepretation} can be decomposed using the new defined partition of the knowledge:
% \begin{equation}
% 	\begin{split}
% 	\by'&= \sigma \left(\bz + \sum_{c \in \G(\clauses_U)} \bdelta_c + \sum_{c \in \G(\clauses_B)} \bdelta_c \right)	
% 	\end{split}
% 	\label{eq:final_intepretation_binary}
% \end{equation}

% Notice that the approach defined in the previous section with a single CE for each clause can be directly applied to the unary knowledge $\clauses_U$. We need to define a strategy to deal with binary clauses. 

% % The idea now is to apply KE to the two sets $\clauses_U$ and $\clauses_B$ separately.
% % % % : the changes to be applied on binary predicates comes only from binary clauses, while the changes on unary clauses depends on both unary and binary clauses.
% % In the first case, KE can be called directly on $\U$ using only the unary knowledge $\clauses_U$ since here all the clauses involves a single variable and only unary predicates (all inside $\U$).
% % % This can be done since $\U$ contains only unary predicates and it represents the data in the same way \TODO{of $\bz$ for the multi-label version of \kenn.} 
% % The output of KE is a matrix that collects the changes to be applied to $\U$ based on unary clauses $\clauses_U$. We call it $\delta \U^u$ to distinguish it from $\delta \U^b$ (the changes to apply to matrix $\U$ based on binary clauses).

% % At this point we also need to increase the satisfaction of binary clauses. To do this, the idea is to reduce the binary case to the unary one so we can still use the KE as defined in Section\TODO{....}. Next sections dive more deeply into this approach.

% \subsubsection{Representing relational data in tables}
% \label{sec:relational_representation}

% To represent relational data, \kenn\ adopts two matrices, denoted by $\U$ and $\B$, which could be seen as tables of a relational database. Fig.~\ref{fig:representation} shows this representation using the classical Smoker-Friends-Cancer example: there is a domain composed of three objects (persons) $O = \{o_0, o_1, o_2\}$, two unary predicates ($S$ and $C$, which stand for $Smoking$ and $Cancer$) and one binary predicate $F$ ($Friends$)). Fig.~\ref{fig:representation}(a) shows the graph representation with nodes and edges labelled with the unary and binary predicates respectively. In this particular example the graph has no self-loops, meaning that $Friends(x,x)$ is not taken into account. Please notice that this limitation is specific for this example since everyone is assumed to be friends of himself a priori. However, in general, \kenn\ can work with self-loops.

% Fig.~\ref{fig:representation}(b) shows the data structure used to encode the graph of Fig.~\ref{fig:representation}(a): matrix $\U$ contains as many rows as objects in the domain and as many columns as unary predicates plus a key column $i$, which could be interpreted as a primary key for the table $\U$. Intuitively, 
% the $j^{th}$ row of $\U$ contains the preactivations of the unary predicates applied on the $j^{th}$ object,
% i.e., $\U_j=(z_{P_1(o_j)},\dots,z_{P_n(o_j)})$. 

% Matrix $\B$ contains one row for every pair of objects to which we want to apply
% a binary predicate. 
% Notice that we might not want to include all the pairs of objects in $\B$, because the application of binary predicates of some pairs might be meaningless. For instance, as already mentioned, the $Friends$ predicate applied to $(a,a)$ is not interesting.
% $\B$ has one column for each binary predicate and other two columns $s^x$ and $s^y$ that indicate the first and the second component of the
% pair. In the relational database analogy they can be seen as foreign keys to table $\U$. As with $\U$, each row represents a different grounding of the predicates, with the difference that in this case the predicates are binary and the variables to be substituted are two. More precisely, $\B_{i,j}$ corresponds to the value of predicate $B_j$ for the substitution $(x / o_{s^x_i}, y / o_{s^y_i})$:
% $$\B_{i,j} = B_j(o_{s^x_i},o_{s^y_i})$$

% For instance, in Fig.~\ref{fig:representation}(b): $s^x_0 = 0$ and $s^y_0 = 1$, which means that row $0$ of matrix $\B$ is referring to the pair of objects $(o_0,o_1)$.


% \begin{figure}
% 	\centering
% 	\input{tikz/rel_representation}
%     \caption{
% 		Relational data representation: in this example, three objects ($o_0$, $o_1$ and $o_2$), two unary predicates ($S$ and $C$) and only one binary predicate ($F$). (a): the graph representation; (b): the representation used by \kenn: matrixes $\U$ and $\B$ can be interpreted as tables of a relational database: $\U$ contains all the groundings of unary predicates and an index column $i$ which correspond to the `primary key' of the table; matrix $\B$ contains the groundings of binary predicates together with columns $s^x$ and $s^y$ which corresponds to ``foreign keys''  to table $\U$.
% 		Values refer to preactivations of atoms' truth values.}
%     \label{fig:representation}
% \end{figure}

% \def\alice{a}
% \def\bob{b}
% \def\chris{c}

% \kenn\ considers unary and binary clauses separately, by adopting two separate instantiations of the KE architecture, namely
% KE$_u$ and KE$_b$. The former computes the contributionsof the clauses in $\clauses_u$ and the latter computes the contributions of the clauses in $\clauses_b$.
% The structure of KE$_u$ and KE$_b$ 
% is the same (shown in the right of Figure~\ref{fig:KE_matrix}). The only difference between the two is that KE$_u$
% takes in input the preactivations on unary predicates in $\U$,
% while KE$_b$ takes in input the preactivations of both unary and binary predicates. Indeed, binary clauses can contain unary predicates and
% we need a method to encode unary predicates as binary.










% \subsubsection{Binary extensions of unary predicates}
% \label{sec:join}
% % \TODO{citare Neural Logic Machines (nel loro caso usano il verbo expand, ma di fatto fanno la stessa cosa... ma su tensori)}
% Given a unary predicate $P$, we define its binary extensions as two binary predicates $P^x$ and $P^y$
% and impose the constraints: 

%   \begin{align}
%     \begin{array}{c}
% P^x(x,y) \leftrightarrow P(x) \\
%       P^y(x,y) \leftrightarrow P(y)
%     \end{array}
%     \label{eq:binarized-unary-predicates}
%   \end{align}
% Intuitively, $P^x$ and $P^y$ are binary predicates that ignore the second and the first input, respectively. For instance, let $Smoker(x)$ be the unary predicate that is true if person $x$ smokes. The binary atom $Smoker^x(x,y)$ corresponds to the sentence: ``The first element of the pair $(x,y)$ is a smoker''.

% For each binary clause, we can substitute the original unary predicates with their binary extensions. For instance, the clause
% $$c: \lnot Smoker(x) \lor \lnot Friends(x,y) \lor Smoker(y)$$
% is converted to
% $$c': \lnot Smoker^x(x,y) \lor \lnot Friends(x,y) \lor Smoker^y(x,y)$$

% It is easy to prove that the truth value of any grounding of $c'$ is the same as the corresponding grounding of $c$:
% $$\Big( Smoker^x(\alice,\bob) \leftrightarrow Smoker(\alice) \Big) \land \Big(Smoker^y(\alice,\bob) \leftrightarrow Smoker(\bob)\Big) \models c[x/\alice,y/\bob] \leftrightarrow c'[x/\alice,y/\bob]$$
% After this transformation, binary clauses can be seen as unary clauses on the domain of pairs of objects on which we can apply KE$_b$. \

% % Notice that while in $c$ there were both unary and binary predicates, in $c'$ all the predicates are binary. This is true for the original domain $O$, but they can be seen as unary predicates if we consider the domain of pairs in $O \times O$. The new solution for the binary knowledge comes exactly from this new perspective: if we extend matrix $\B$ to contain also the new binary predicates $U_i^x$ and $U_i^y$, then we can apply directly the KE on the resulting matrix using $\clauses_B$. 

% % In the relational database analogy, this approach is equivalent to perform a JOIN query on $\U$ and $\B$ and apply the KE on the resulting matrix:

% % \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% % 	*$\M$* = SELECT *$s^x$*, *$s^y$*, *$U_i^x$*, *$U_i^y$*, *$B_j$* 
% % 	     FROM U AS Ux, U AS Uy, B
% % 	     WHERE Ux.*$i$* = B.*$s^x$* AND Uy.*$i$* = B.*$s^y$*
% % \end{lstlisting}
% % where $U_i^x$ is a shortcut for selecting all the unary predicates in Ux
% % (Ux.$U_i$ AS $U_i^x$).

% \begin{figure}[t]
% 	\centering
% 	\input{tikz/JOIN}
%     \caption{The JOIN query: all the binary predicates (including the binary extensions) are collected in a unique matrix. The red numbers are all referring to the same grounded atom $C(o_0)$.}
%     \label{fig:join}
% \end{figure}


% % \TODO{
% % Mapping function just need to return a matrix $\M$ which has a row for each pair of objects and a column for each binary predicate (including the binary extensions $U_i^x(x,y)$ and $U_i^y(x,y)$).}

% \subsection{Relational Data - \kenn\ architecture}
% \label{sec:groupby}


% To cope with ``binarized'' unary atoms, table $\B$ is extended with additional columns for the predicates $P^x_i$ and $P^y_i$ for every unary predicate $P_i$. In order to satisfy the constraints in \eqref{eq:binarized-unary-predicates} the values of these new attributes are computed by joining $\B$ and $\U$ on the indexes $i$, $s^x$ and $s^y$. We denote with $\M$ the result of this join:
% \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% 	*$\M$* = SELECT *$s^x$*, *$s^y$*, *$U_i^x$*, *$U_i^y$*, *$B_j$* 
% 	     FROM U AS Ux, U AS Uy, B
% 	     WHERE Ux.*$i$* = B.*$s^x$* AND Uy.*$i$* = B.*$s^y$*
% \end{lstlisting}
% where $U_i^x$ is a shortcut for selecting all the unary predicates in Ux
% (Ux.$U_i$ AS $U_i^x$).



% % we use the so called \emph{mapping function}, which maps the graph representation into a single matrix $\M$. 
% {%\color{red}
% The matrix $\M$ defined by the JOIN query is used by KE$_b$ with $\clauses_B$. KE$_b$ returns $\delta \M$, a table of the same shape (and same values for $s^x$ and $s^y$) of $\M$. Such table contains the changes on the initial predictions induced by binary clauses. Figure~\ref{fig:join} shows an example of the application of join and KE$_b$.}


% Finally, the different delta values associated with each grounded atom are aggregated together. This can be achieved by the following three queries:

% \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% 	*$\delta B$* = SELECT *$\delta B_i$*
% 	     FROM *$\delta M$*
	
% 	*$\delta U_x$* = SELECT SUM(*$\delta U_i^x$*)
% 	      FROM *$\delta M$*
% 	      GROUP BY *$s^x$*

% 	*$\delta U_y$* = SELECT SUM(*$\delta U_i^y$*)
% 	      FROM *$\delta M$*
% 	      GROUP BY *$s^y$*
% \end{lstlisting}

% \noindent Figure~\ref{fig:groupby} shows the second query, which is used to calculate the $\delta U_x$. 

% \begin{figure}[H]
% 	\centering
% 	\input{tikz/GROUP_BY}
% 	\caption{An example of a GROUP BY query: for each unary predicate ($S$ and $C$), the values of their first binary extension ($S^x$ and $C^x$) are summed up based on the index 
% 	% \TODO{Dovrei mettere anche la select e renderla piu chiara???}
% 	}
%     \label{fig:groupby}
% \end{figure}


% \noindent The final preactivations $\U'$ and $\B'$ are
% $$\U' = \U + \delta \U_u + \delta \U_x + \delta \U_y$$
% and
% $$\B' = \B + \delta \B$$



% % the \emph{reverse mapping function} takes in input $\delta \M$ and outputs $\delta \U^b$ and $\delta \B$ which are added to $\U$ and $\B$ to obtain the final predictions.}

% \noindent Figure~\ref{fig:unary_binary} shows a high-level overview of the entire model.

% % In the next chapter, the implementation details will be introduced, with a focus on how to implement the four queries introduced in this chapter as differentiable functions.


% \begin{figure}
% 	\centering
% 	\input{tikz/rel_overview}
% 	\caption{
% 	To obtain $\delta \U_u$, unary clauses $\clauses_U$ are used by KE directly on $\U$. The JOIN query is used to find matrix $\M$. Then, the KE is applied to $\M$ using binary clauses $\clauses_B$. Finally, to obtain $\delta \U_b$ and $\delta \B$ other three queries are used.}
%     \label{fig:unary_binary}
% \end{figure}




% \subsection{Knowledge for inputs/outputs relationships}
% \label{sec:KENN_inputs}
% Until now, we defined \kenn\ as a method that injects logical knowledge which represents relationships between different predictions of a Neural Network. However, it is even possible to provide knowledge which expresses relationships between inputs and outputs values. In other words, if some of the inputs are truth values of some atomic formulas, we can add clauses that contain them, providing in this way information on the relations between inputs and outputs. 

% Figure~\ref{fig:KENN_inputs} introduces this idea: the solution is straightforward, we just need to concatenate the inputs of the base NN with its outputs before applying the KE. The KE will provide an updated version of both inputs ($\bx'$) and outputs ($\by'$). Since we are interested only in the outputs, the last step discards the changed inputs $\bx'$.

% \begin{figure}[H]
% 	\centering
% 	\input{tikz/KENN_inputs}
% 	\caption{KENN used with knowledge on both inputs and predictions: the ``preactivations'' $\bz_x$ of inputs $\bx$ are calculated with the logit function and concatenated to the preactivations of the outputs $\by$. The result can be used by KE to force the satisfaction of the knowledge.}
% 	\label{fig:KENN_inputs}
% \end{figure}

% Notice that, since the KE works with preactivations, the logit function (the inverse of logistic function) must be applied to the inputs before the concatenation. Moreover, the logit is defined in the range $(0,1)$, which means that if the truth values in $\bx$ are zeros and ones, logit can not be applied directly. For this reason, a small number $\epsilon$ is added or subtracted to $\bx$ before applying the logit. Alternatively, $\bz_x$ can be set to a high value when $\bx$ is positive and a very high negative number when it is negative (in our experiments we used 500 and -500).
% %  to keep the values of $\bx$ in the domain of the logit function.

% % \section{Mapping function}
% % \TODO{spostare in implementazione e sistemare}
% %  The mapping function makes use of \emph{gather} function of TensorFlow which slices a given matrix according to an indices vector. In Fig.~\ref{fig:gather} an example of \emph{tf.gather} usage. For more details about \emph{tf.gather} see the official \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation}.

% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/gather_example}
% %     \caption{\emph{tf.gather} behaviour: given a matrix $\U$, it copies in a new matrix the rows of $\U$ based on the provided indices.}
% %     \label{fig:gather}
% % \end{figure}

% % Vectors $s^x$ and $s^y$ contain the indexes of the objects in $\U$ which are referred by matrix $\B$. For instance, in Fig.~\ref{fig:gather} $s^y_0=1$, which means that in the first row of $\B$ the $y$ variable of the binary predicates is substituted by object $\bob$ . Therefore, when \emph{tf.gather} is applied to $\U$ using $s^x$ ($s^y$) it generates a matrix containing the values of $U_i^x$ ($U_i^y$) corresponding to the grounding in $\B$. The mapping function just need to concatenate the resulting matrices with $\B$ to obtain the final matrix $\M$. Fig.~\ref{fig:mapping}~shows the implementation of mapping function.

% % The key point of this strategy is that we can apply the KE on matrix $\M$ using $\clauses_B$. The result $\delta \M$ is a matrix of the same shape of $\M$ which collects all the changes to be applied on atomic formulas due to binary clauses.

% % Now we just need to define the reverse mapping function, which copies $\delta \M$ values into the initial representation: it returns the final changes (generated from $\clauses_B$) that should be applied on unary ($\delta \U^b$) and binary ($\delta \B$) grounded predicates.

% % % to copy the unary predicates in the right spots of final matrix $\M$ (see \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation} for a better description of \emph{tf.gather} function).

% % % In the shown example:
% % % $$
% % % s^x = \ensuremath{\begin{pmatrix}0\\0\\1\\1\\2\\2\end{pmatrix}}
% % % $$

% % % This is telling us that the first two rows of matrix $\B$
% % % % and of the final matrix $M$
% % % are referring to the object in row $0$ of $\U$, while the third and fourth row correspond to row $1$ in $\U$. By applying \emph{tf.gather} to matrix $\U$ and vector $s^x$ we generate a matrix which contains the unary predicates values for the objects referred by $s^x$. The same strategy is applied with $s^y$. Finally we concatenate the two resulting matrices with $\B$. The final matrix $\M$ can be seen as an extension of matrix $\B$ obtained by adding the missing binary predicates (the binary extensions of unary predicates). 



% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/rel_mapping}
% %     \caption{\TODO{usare anche qui l'esempio, specificare almeno una regola logica e mettere dei valori sensati..., aggiungere altra immagine separate per l'applicazione del KE (sempre con lo stesso esempio) in cui si mostra esattamente cosa succede} The architecture of mapping function: it applies \emph{tf.gather} to $\U$ using as indices $s^x$ and $s^y$. The resulting matrices contain $\U$'s rows ordered as specified by the two vectors. Finally, using the concatenation it generates matrix $\M$ which can be provided as input to the KE together with the binary knowledge $\clauses_B$.}
% %     \label{fig:mapping}
% % \end{figure}



% % \section{Reverse mapping function}
% % \label{reverse}
% % \TODO{spostare in implementazione e sistemare}

% % From Fig.~\ref{fig:mapping} we can notice that we have multiple delta values for each grounded unary predicate inside matrix $\delta \M$. For instance, the values of $M_{0,2}$, $M_{2,0}$, $M_{3,0}$ and $M_{5,2}$ are all referring to $U_1(\bob)$ and they come from different grounding of the binary clauses.

% % The reverse mapping function works in reverse of the mapping function. The first step is to split $\delta \M$ in three matrices: $\delta \M^x$ contains the delta values for predicates of the form $U_i^x$, $\delta \M^y$ refers to predicates $U_i^y$ and $\delta \B$ to binary predicates $B_j$. 

% % % \AD{Notice that $\delta \M^x$ does not contain any predicates that refers to variable $y$ (the same is true for $\delta \M^y$ and variable $x$). Therefore, we can see the predicates referred by $\delta \M^x$ as the original unary predicates (instead of using their binary extensions). Indeed, $\delta \M^x$ has a similar structure as $\U$, with the exception that multiple rows refer to the same object.}

% % The proposed changes for binary predicates ($\delta \B$) are already usable. In other words, they can be directly added to matrix $\B$ to obtain final preactivations $\B'$: 
% % $$\B' = \B + \delta \B$$

% % For the unary predicates it is needed an additional step: we have to collect all the changes referring to the same atomic formula, sum them together and put the results in the right position of matrix $\delta \U^b$. This is achieved through the use of \emph{scatter\_nd} function of TensorFlow which works in reverse of \emph{tf.gather}. Indeed, while for \emph{tf.gather} the indices refer to the input matrix, with \emph{tf.scatter\_nd} they refer to the output matrix. Fig.~\ref{fig:scatter} shows an example of \emph{tf.scatter\_nd} usage (see \href{https://www.tensorflow.org/api_docs/python/tf/scatter_nd}{TensorFlow documentation} for more details). Notice that when the indices vector contains multiple indices with the same value, the corresponding rows are summed together before being copied. 

% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/scatter_example}
% %     \caption{\emph{tf.scatter} behaviour: it copies the rows of a matrix in the specified indices. When multiple indices are equivalent it sums the corresponding rows.}
% %     \label{fig:scatter}
% % \end{figure}

% % Using \emph{tf.scatter\_nd} with indices vector $s^x$, \kenn\ can automatically sum up all the contributions of the same atomic formula found in $\delta \M^x$ and put the results in the right position inside a new matrix called $\delta \U^x$. The same strategy is applied for calculating $\delta \U^y$ matrix. Then the two matrices are summed together to obtain $\delta \U^b$:
% % $$\delta \U^b = \delta \U^x + \delta \U^y$$
% % Finally, the preactivations of unary predicates are calculated as:
% % $$\U' = \U + \delta \U^u + \delta \U^b$$

% % The detailed architecture of the reverse mapping function can be seen in Fig.~\ref{fig:reverse_mapping}.


% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/rel_reverse_mapping}
% %     \caption{\TODO{Continuare anche qui con l'esempio solito} The architecture of the reverse mapping function: first, it splits $\delta \M$ into three matrices which contain the improvements to apply to predicates $U_i^x$, $U_i^y$ and $B_i$. It then makes use of \emph{tf.scatter\_nd} to add all the values referring to the same atomic formulas and store them in the right position in $\delta \U^x$ and $\delta \U^y$. Finally, the two matrices are added together to obtain $\delta \U^b$.}
% %     \label{fig:reverse_mapping}
% % \end{figure}


% % % \begin{figure*}
% % %     \makebox[\textwidth][c]{
% % %         \includegraphics[scale=0.09]{reverse_mapping.jpg}
% % %     }
% % %     \caption{The reverse mapping function projects the changes proposed by KE (with binary clauses $\clauses_B$) into the original data structure of the underlying graph. It makes use of \emph{tf.scatter\_nd} function, which works in reverse as \emph{tf.gather}: it sums up all the rows in $\delta \U^x$ that refer to the same object in $O$. In other words, it sums rows with the same value in $s^x$. The same is done for $\delta \U^y$ and $s^y$. The final matrices has the same shape as $U'$ and they are summed to it to obtain the final unary predictions $U$.}
% % %     \label{fig:reverse_mapping}
% % % \end{figure*}





% % {


% % % \begin{TODO LIST}{TODO}
% % %     \item Aggiungere spiegazione formale del perche' e' corretto (scatter\_nd calcola la somma su tutti i groundings...)
% % %     \item aggiungere in appendix descrizione di scatter\_nd e gather
% % % \end{TODO LIST}


% % }




% % % \TODO{
% % % Figure~\ref{fig:CE} shows in details the architecture of \kenn's last layer. KE is a function that takes as input the preactivations ${\bz}$ of the base NN and produces the final activations ${\by'}$. In the picture, $\bz$ is visualized as a vector. However, in the general case it is a matrix whose columns represents a predicate and each row an object. In other words, element $z_{ij}$ represents the preactivation of $P_j(o_i)$, where $P_j$ is the $j^{th}$ predicate, and $o_i$ the $i^{th}$ object. This representation restricts the scenarios where we can apply \kenn: it can be used in the context of multi-label classification, but it is not straightforward to use it in the presence of both unary and binary predicates. In Chapter~\ref{ch:srl} we will see how to extend \kenn \ to work with relational data as well.



% % % Internally, for each clause $c \in \clauses$, KE has a sub-module called \emph{Clause Enhancer} (CE), which returns $\delta_c^z$, the adjustments to be applied on preactivations to enforce $c$ satisfaction. Such values are also stored in a matrix of the same shape of $\bz$. In this way it is easy to aggregate all the contributions for different clauses: CEs outputs are combined linearly using \emph{clauses weights} and summed to the initial preactivations.}

% % % Lastly, the final predictions are calculated by applying the logistic function:

% % % \TODO{
% % % \begin{equation}
% % %   \label{eq:ke}
% % %   y'_i = \sigma\Big(z_i + \sum_{c \in \clauses \atop i \in c} 
% % %   \sign_{c,i}\cdot \delta^{w_c}_s(\bsign_c\odot {\bz}_c)_i \Big)
% % % \end{equation}

% % % Cambiare formula (usando la notazione precedente): la predizione di una formula atomica e' la somma tra la predizione iniziale e la somma dei vari delta generati dai CE... (riferirsi a questa formula dopo, nell'implementazione (dove si deve mostrare che effettivamente e' quello che otteniamo usando la matrice z e gather) e nella parte relazionale (in quel caso si deve distinguere tra predicati unari e binari e mostrare che con mapping e reverse mapping otteniamo esattamente quello che vogiamo))}

% % % \noindent where $i\in c$ means that the clause $c$ contains a positive or negative literal corresponding to the preactivations $z_i$, $\bz_c$ are all the preactivations corresponding to the literals in $c$, $\odot$ is the element-wise multiplication, and $\bsign_c$ is a polarity vector of $1$ and $-1$, with $\sign_i=1$ if the $i^{th}$ literal of the clause is positive and $\sign_i=-1$ if it is negative.

 

% % % \chapter{KENN for Statistical Relational Learning}\label{ch:srl}

% % % % \newcommand{\ad}[1]{{\color{blue}#1}}

% % % \begin{TODO LIST}{TODO}
% % %     \item Espandere descrizione:
% % %     \begin{itemize}
% % %         \item Far capire perche la prima versione di \kenn \ non puo essere usata coi dati relazionali (facendo riferimento anche al nuovo capitolo sull'implementazione)
% % %         \item Concantrarsi sul l caso con regole n-arie, e specificare in seguito che nella partica si arriva di solito a arieta 2 o 3 e che ho testato solo con 2 (esempio e immagine con arieta' 2 per semplicita di esposizione)
% % %         \item Usare l'esempio pratico dei documenti (per tutto il capitolo fare riferimento a tale esempio, mostrando come a partire dalle previsioni iniziali e dalle regole logiche si arrivi alle predizioni finali)
% % %         \item Far capire come i vettori di indici sono passati
% % %         \item mettere in chiaro che gli indici possono essere passati dell'utente finale (per esempio, in riferimento all'immagine della rappresentazione, non ci sono self loop nel grafo... questo solo perche il grafo da rappresentare non aveva self loops)
% % %         \item Aggiunta dimostrazione formale del fatto che con mapping e reverse mapping i delta finali sono ancora la somma dei vari delta su tutti i grounding delle regole logiche (dimostrazione divisa in predicati binari e predicati unari) e di conseguenza si soddisfa la formula introdotta nel capitolo teorico su \kenn
% % %         \item [opt] many sorted logic: aggiungendo una tabella per ogni dominio e usando piu volte la mapping function e la reverse su diverse tabelle e' possibile in teoria gestire diversi domini...\\
% % %         In tal caso, per ogni termine di un predicato si definisce il dominio (come in PSL)
% % %     \end{itemize}
% % % \end{TODO LIST}

% % % \begin{TODO LIST}{TODO}
% % %     \item Aggiunta dettagli implementativi
    
% % % \end{TODO LIST}

% % % The first version of \kenn\ has been developed for multilabel classification. \AD{In this chapter we are interested in extending \kenn\ for relational data, where the single matrix representation introduced in Section~\ref{sec:architecture} can not be used.


% % % Such representation is exploited by \kenn\ to minimize the required computational effort: all the operations can be expressed as matrix operations, which are 
% % % Such representation has an advantage: all the Knowledge Enhancer's internal calculations are implemented as matrix operations, which are particularly efficient when working with a GPU. However, the usage of $\bz$ is limiting since it is not possible to represent both unary and binary predicates in such matrix.
% % % and we would like for \kenn\ to consider also binary predicates, which is not possible with the matrix representation we have seen so far.

% % % \AD{
% % % Although the ideas behind \kenn\ could be applied to other types of tasks,the current implementation requires to represent data in a particular format. For this reason, it is not straightforward to use it in different contexts other than multi-label classification.
% % % }

% % % \TODO{
% % % Although the ideas behind \kenn\ could be applied to other types of tasks, the current implementation requires to represent data in a particular format, which is exploited by \kenn\ implementation to minimize the required computational effort. For this reason, \kenn\ can be applied for solving multi-label classification tasks, but it is not straightforward to use it in different contexts. }

% % % More in details, in the architecture introduced in Section~\ref{sec:architecture}, atomic formulas preactivations
% % % % to be modified
% % % are stored as elements of a matrix $\bz$.
% % % %  with columns representing predicates and rows the \TODO{groundings}. 
% % % \AD{Each column of $\bz$ refers to a unary predicate and each row refers to a specific object of the domain. All the atomic formulas in the row are obtained by substituting the free variable of a unary predicate (the one corresponding to the column) with that object.} Such representation is limiting and we would like for \kenn\
% % % % to be more flexible on the data structure used to store atomic formulas' values. We would like 
% % % to consider also binary predicates,\ which is not possible with the matrix representation we have seen so far.
% % % % \TODO{(spostare) each row of $\bz$ refers to a specific object of the domain and all the atomic formulas in the row are obtained by substituting the free variable of a unary predicate with that object.}

% % % We want to extend \kenn\ to work with graphs: instead of focusing only on unary predicates we need to use binary predicates as well. 
% % % The next sections introduces the extension of \kenn\ for relational data, which can be applied on graphs.
% % %  mantaining the good time performances obtained by the usage of the single matrix representation. 
% % % In designing this extension I paid particular attention to maintain the computational efficiency we have obtained in the previous version.}


% % %it would be preferable to keep the good time performances obtained by the usage of the single matrix representation. 


% % % \TODO{
% % % The idea is to develop a mapping function $m$ which can convert a custom representation into the matrix representation used so far. Moreover, we need a reverse mapping function $r$ which converts back the results to the required representation. In this way, we could keep the same implementation of KE.

% % % (reduce the graph problem to the original one...)




% % % % \begin{figure*}
% % % %     \makebox[\textwidth][c]{
% % % %         \includegraphics[scale=0.4]{imgs/m.jpg}
% % % %     }
% % % %     \caption{\kenn\ architecture: (a) for multilabel classification; (b) with structured NN output}
% % % %     \label{fig:mapping}
% % % % \end{figure*}


% % % In Fig.~\ref{fig:mapping}(a) it is shown the original version of \kenn: a neural network (NN) returns preactivations $\bz'$ based on features $\bx$, then \emph{Knowledge Enhancer} (KE) function takes $\bz'$ as input and returns $\delta \bz$, the update to be added to $\bz'$ in order to obtain the final preactivations $\bz$ (which in turn will be feed to the logistic function). Notice that the image is slightly different from the one of the original paper where the sum between $\bz'$ and $\delta \bz$ were performed inside KE together with the application of logistic regression. However, for the sake of this document, this representation is more useful.

% % % In Fig.~\ref{fig:mapping}(b) it is shown a new version of \kenn: here the results of the neural network have a different representation. Before applying KE, we use mapping function $m$ to store NN predictions into a matrix $M$ that can be processed by KE. A reverse mapping function $r$ is used to change the representation of KE outputs $\delta \M$ (changes to be applied to initial predictions) into the original representation and only then $\bz'$ and $\delta \bz$ are combined (notice that we require the addition to be defined for such a representation).


% % % }
% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "paper KENN"
% %%% End:


==> Relational KENN/collective.tex <==


\section{Evaluation of the model}\label{sec:collective}

In this section, the relational extension of \kenn\ is tested on the task of Collective Classification: given a graph,
we are interested in finding a classification for its nodes using both features of the nodes (the objects) and the information coming from the edges of the graph (relations between objects)~\cite{collective_classification}.

In Collective Classification, there are two different learning tasks: inductive and transductive learning. In inductive learning, there are two separate graphs, one for training and the other for testing. On the contrary, in transductive learning, there is only one graph that contains nodes both for training and testing. In other words, in inductive learning, there are no edges between nodes for training and testing, while in transductive learning there are. 
% Figure~\ref{fig:collective} shows the difference between the two paradigms.
% \begin{figure}
% 	\centering
% 	\input{tikz/inductive_transductive.tex}
%     \caption{The two learning paradigms in Collective Classification. The colors represent the classes of the nodes. White nodes are nodes of the Test Set. In inductive learning, Training and Test sets are two distinct graphs: the network has to learn only from labeled data; in transductive learning, there is a unique graph with both training and test nodes: the network can make use of information coming from the Test Set at training time by considering the additional relations.}
%     \label{fig:collective}
% \end{figure}
% \TODO{....estendere.... The ML algorithm has to learn to generalize to new graphs.  ....on transductive learning where the goal is to provide predictions only of unlabelled data that is available at training time~\cite{zhu, yang}. 
The tests have been performed on both tasks \new{to analyze the behavior of \kenn\ in the contexts of relational domains. In particular, we tested \kenn\ with a varying number of KEs layers to validate the proposal of Section~\ref{sec:reasoning}.\footnote{Source code of the experiments are available on \href{https://github.com/rmazzier/KENN-Citeseer-Experiments}{https://github.com/rmazzier/KENN-Citeseer-Experiments}
}. }
% To maintain anonymity, we provide it in the supplementary materials. This footnote will contain the url in the final submission.
% at \href{https://github.com/rmazzier/KENN-Citeseer-Experiments}{https://github.com/rmazzier/KENN-Citeseer-Experiments}
% }.


\subsection{Experimental setup}
\label{sec:exp_setup}
We followed the evaluation methodology of~\cite{RNM}, where the experiments have been carried out on Citeseer dataset~\cite{citeseer} using SBR and RNM. 
The Citeseer dataset used in the evaluation is a citation network: the graph's nodes represent documents and the edges represent citations. The nodes' features are bag-of-words vectors, where an entry is zero if the corresponding word of the dictionary is absent in the document, and one if it is present. The classes to be predicted represent possible topics for a document.
The dataset contains 3312 nodes that must be classified in 6 different classes: AG, AI, DB, IR, ML, and HCI.
%  \TODO{mettere nomi per intero}.
The classification is obtained from the 3703 features of the nodes, with the addition of the information coming from the citations (4732 edges).

% As in~\cite{RNM}, the experiments have been performed on both inductive and transductive paradigms

% \new{Moreover, we tested \kenn\ at varying the number of KEs layers on top of the model. } 
\new{
    % Moreover, 
We use the same NN and knowledge as in~\cite{RNM}, allowing for the comparison with SBR and RNM.}
% , meaning that the results of \kenn\ \todo{are directly comparable} with the results of SBR and RNM.} 
% More in detail, we use as 
The NN is a dense network with 3 hidden layers, each with 50 hidden nodes and ReLU activation function. 
\new{The knowledge consists of six rules obtained by substituting the topic $T$ in $
\lnot T(x) \lor \lnot Cite(x,y) \lor T(y)
$ with all the classes, and they codify the idea that papers cite works that are related to them. 
% This implies that the topic of a paper is often the same as the paper it cites.
}

% The prior knowledge codifies the idea that papers cite works that are related to them. This implies that the topic of a paper is often the same as the paper it cites. The clause
% $
% \lnot T(x) \lor \lnot Cite(x,y) \lor T(y)
% $
% is instantiated multiple times by substituting the topic $T$ with all the six classes.


% multiple evaluations have been made while changing the amount of trained data.

% We evaluated \kenn\ with the same settings as \cite{RNM}, where SBR and RNM where trained with different percentage of dataset for the training set. \TODO{In this way, we obtain a comparison with SBR }

% \TODO{
% using \TODO{Citeseer~\cite{collective_classification}}, a collective classification dataset. In the task of collective classification .}


% \TODO{dopo.....??.. We focus on semi-supervised node classification, where labels are provided for a small subset of the graph and the model is trained using both labelled and unlaballed data. }



% \subsection{Citeseer Dataset\todo{unificare con sezione successiva (experimental setup)?}}


% \subsection{The prior knowledge}


% \subsection{Bibliography Knowledge}
% \AD{Notice that the above axioms assume that one paper cites only papers of the same topic. In most of the cases this is not true. For instance, if the graph is fully connected the aximos are true only if all the papers are about the same topic. For this reason we propose a softer version that consider the topic of the bibliography as a whole.

% The new type of knowledge, called Bibliography Knowledge, defines a new unary predicate $T_B$ for each topic $T$.} Intuitively, $T_B(x)$ should be true if the bibliography of paper $x$ can be classified as topic $T$.

% For each topic, we define the clause:
% $$
% \forall x \ T_B(x) \to T(x)
% $$
% \noindent meaning that a paper must be classified with the same topic of its bibliography.

% To calculate this bibliography predicates the model first multiplies the predictions of the NN for the adjacency matrix of the citation graph and then it applies the softmax function to each row of the resulting matrix:
% $$
% \T^B = softmax(\A \T)
% $$
% \AD{
% \noindent where $\T$ is the matrix containing the topics for each paper as predicted by the GCN (similar to the definition of $\bz$, each colum represents a topic and each row a node of the graph); $\A$ is the adjacency matrix of the citation graph: it contains all the citations between papers and is defined as the matrix with values $A_{ij} = Cite(o_i,o_j)$.
% }





% \todo{(togliere?) Notice that the NN takes as input only the features of the nodes and it does not take into account relations. For this reason, by adding the knowledge, we could expect improvements as compared to the NN. Notice also that for the NN model the two paradigms (inductive and transductive) are equivalent: the only
% difference between the two is the presence or absence of relations between nodes in the training and test sets, and such relations are not taken into account by the NN. For this reason, we used the same initialization of the NN weights in both inductive and transductive learning (using the same seed). Indeed, the predictions of the NN are the same in the two cases, while}



% Notice also that the citations are known a priori (the edges of the graph are given as inputs). Therefore, when applying KE, it is possible to focus only on pairs of documents for which the $Cite(x,y)$ predicate is known to be true. Indeed, all the grounded clauses in the Prior Knowledge are automatically satisfied if $Cite(x,y)$ is false for the specific grounding. This means that clauses are always satisfied when the pair of documents do not cite one another and that KE would not apply any changes for such pairs of objects. For this reason, $s_i^x$, $s_i^y$ and $\B$ were generated using only pairs of objects for which $Cite(x,y)$ is true, reducing both train and test time. 

% Finally, since each paper can not be classified with multiple classes, the activation used was the $\softmax$ function. Notice that the results obtained in Section~\ref{preact} were proved with the assumption that the activation is a logistic function. Therefore, there is not theoretic evidence that this approach can work. However, the results obtained give us empirical evidence that \kenn\ can improve the NN predictions even with $\softmax$ activation.

The training set dimension is changed multiple times to evaluate the efficacy of the three methods on the varying of training data. More precisely, tests have been conducted by selecting 10\%, 25\%, 50\%, 75\%, and 90\% of nodes for training. For each of these values, the training and evaluation were performed 100 times, each with a different split of the dataset. At each run the training set is created by selecting random nodes of the graph, with the constraints that the dataset must be balanced.
%  (i.e., each of the 6 classes has the same amount of nodes in the training data).

% \todo{(cambiare)
% In~\cite{RNM}, the number of runs was ten for each percentage of training data and the final results were obtained as the mean of accuracy in those ten runs. This was justified by the fact that the choice of nodes in the Training Set has a strong effect on the learned model, and as a consequence on the test accuracy. However, during our experiments, we noticed that the standard deviations of both NN and KENN's results were rather high. As a consequence, when running multiple times the 10 iterations, the results were much different every time. For this reason, differently from~\cite{RNM}, for each training dimension we performed 500 \todo{100?} runs instead of 10.}

% \todo{Aggiungere anche il discorso del cambio del numero di KE layers}

%This was necessary to provide meaningful results since at each step the training/validation/test split is randomly generated and, as a consequence, the results present high variance.

% \new{Finally, to evaluate the relevance of our results we calculated the p-values for each percentage of training data, where the considered null Hypothesis corresponds to the supposition that the distribution of accuracies of the NN is the same as KENN.}
%  In other words, we calculated the probability of obtaining our results under the assumption that the additional knowledge injected by KENN is not helpful.
% Moreover, for each experiment, we calculated a 99\% confidence interval on the improvements obtained by KENN.


% For each of this values, the training set is created 10 times and both \kenn\ and the NN are trained on all versions. The final results are calculated as the average of the results in the ten cases. This is done also in~\cite{RNM} and the reason is that the choice of the training nodes deeply affect the results.

% 

% \TODO{10 run e media}

\subsection{Results}
\label{sec:results}
\begin{figure}
    \centering
    % \makebox[\textwidth][c]{
        \includegraphics[scale=0.35]{plots/n_layers_plot.png}
    % }
    \caption{\new{Accuracies of \kenn\ at the varying of KEs layers.
    %  Each line is associated with a different percentage of training samples and it is surrounded by a 99\% confidence interval.
    }}
    \label{fig:comparison_n_layers}
\end{figure}

\new{Figure~\ref{fig:comparison_n_layers} shows the test accuracies obtained by \kenn\ while increasing the number of KEs layers, starting from $0$ (corresponding to the NN accuracy) up to 6. Note that, for each line in the figure, there is a surrounding border corresponding to a 99\% confidence interval.
% Note that for each result we have calculated a 99\% confidence interval, which is shown in the figure as a border surrounding the corresponding line. 
To calculate the intervals, we assumed the distribution of improvements obtained by the injection of the logical rules to be a normal distribution (see figures in Appendix B and C).
%  Given this assumption, w
We also computed the p-values for each setting, assuming as null Hypothesis 
% where the considered null Hypothesis corresponds to the supposition 
that the distribution of accuracies of the NN is the same as \kenn. Since the number of runs, as well as the obtained improvements, are quite high, the resulting p-values are very small. For this reason, we can safely reject the null Hypothesis, and we are very confident that the improvements given by \kenn\ do not depend on the random initialization of the models' parameters or the specific choices of the splits of the dataset.}

\new{More in detail, we found p-values in the range from 8.2e-42 to 1.6e-09 in the inductive case, and from 53e-72 to 2.1e-23 for the transductive one. The only exception is with 90\% of the samples in the inductive scenario where the p-value is 0.35. This is because the improvements over the NN are very small. Indeed, in both learning paradigms, the effect of the knowledge is reduced when the amount of available data is larger. This behavior is consistent with the simple intuition that, when the training data is scarce, the usage of knowledge should bring higher benefits.
} 

\new{A more important result coming from these experiments is the fact that in all cases adding a new KE layer does not reduce the test accuracy. On the contrary, most of the time the metric is increased until a certain number of layers is reached, and after that, the accuracy stabilizes. This behavior is in line with the discussion of Section~\ref{sec:reasoning} and confirms the efficacy of the proposed strategy to deal with the violation of independece assumption. }

% \todo{
% Moreover, note that in the transductive case the improvements ... by the usage of the knowledge are higher. Indeed, ...}

\new{
Finally, Figure~\ref{fig:comparison_n_layers} provide also a measure of the amount of information carried out by the knowledge. For instance, consider blue and yellow lines, corresponding to a training set with 25\% and 50\% of the samples, respectively. In the inductive scenario, the accuracy obtained with 25\% with the addition of the knowledge is almost the same as the standard NN with 50\% of the data (even higher in the transductive scenario). In this case, adding the knowledge has the same effect of doubling up the training data! Indeed, one of the main motivations behind Neural-Symbolic Integration consists in reducing the required amount of training samples since collecting labeled data is costly in practice.
}





% More in detail, the p-values are all in the range from 8.2e-42 (for 25\% of the training data) to 1.6e-09 (in the case of 75\%). \new{for inductive learning and even smaller in the transductive case .} 


\subsection{Comparison with other NeSy frameworks}
\label{sec:comparison}
\new{Table~\ref{tab:comparison} shows a comparison of \kenn\ with SBR and RNM. We used the results of \kenn\ with 3 KEs since more layers do not provide a significant advantage (see Section~\ref{sec:results}).
}

\begin{table}[H]
    \caption{Improvements in terms of accuracy on inductive and transductive learning. 
    % The first three columns contains the results reported in~\protect\cite{RNM}.
    }
    % , while my results are in the last three. Notice that the NN results are slightly different in the two versions}
    \centering
    \begin{tabular}{c|lll|lll}
        \multicolumn{4}{c}{\ \ \ \ \ \ \ Inductive} & \multicolumn{3}{c}{Transductive} \\
        \rule{0pt}{2ex}\hspace{-0.12cm}
        \% Tr & SBR & RNM & \kenn & SBR & RNM & \kenn \\
        \hline
        \rule{0pt}{2ex}\hspace{-0.12cm}
        10 & 0.005 & 0.040 & {\bfseries 0.052} & 0.063 & 0.068 & {\bfseries 0.110}\\
        \rule{0pt}{1.5ex}\hspace{-0.12cm}
        25 &  0.008 & 0.035 & {\bfseries 0.044} & 0.062 & 0.068 & {\bfseries 0.074}\\
        \rule{0pt}{1.5ex}\hspace{-0.12cm}
        50 & 0.005 & 0.019 & {\bfseries 0.036} & 0.052 & 0.058 & {\bfseries 0.064} \\
        \rule{0pt}{1.5ex}\hspace{-0.12cm}
        75 & 0.002 & 0.009 & {\bfseries 0.021} & 0.056 & {\bfseries 0.058} & 0.057 \\
        \rule{0pt}{1.5ex}\hspace{-0.12cm}
        90 & 0.003 & {\bfseries 0.009} & 0.001 & {\bfseries 0.054} & {\bfseries 0.054} & 0.043\\
        \hline
        \hline
    \end{tabular}
    \label{tab:comparison}
\end{table}

\new{As we can see from the table, in the inductive case SBR produces much lower improvements compared to the other two methods.} Note that these results are in line with previous results obtained on VRD dataset, where another regularization approach (LTN) was compared with KENN~\cite{kenn}. Indeed, the results obtained in both VRD and Citeseer suggest better performances of model-based approaches as compared to the ones based on regularization. 
% This could be explained by the ability of model-based methods to adapt to partially unsatisfied constraints by learning clause weights. 
Note that methods based on regularization of the loss do not impose the knowledge at inference time. In the transductive scenario, the situation is different and SBR behaves similarly to the other two. Indeed, in this case, citations between training and test nodes are available and there is no distinction between training and inference.


% Moreover, the behavior of \kenn\ and RNM is consistent with the simple intuition that, when the training data is scarce, the usage of knowledge should bring higher benefits.
% %  \TODO{That is because the knowledge becomes redundant when the amount of data is large enough and the NN can implicitly learn the given rules directly from the Training Set.}
% Indeed, the two methods produce large improvements in the smaller datasets and such improvements decrease when adding more samples to the Training Set.
\new{
Finally, the results suggest that \kenn\ is particularly useful when the training data available is scarce. On the contrary, when data is abundant, our results tend to degrade faster than RNM and SBR.
% To deal with these problems, it optimizes the satisfaction of the constraints defined by the knowledge even at test time \todo{collective classification (citazione)}. This is a strong point in favor of \kenn\ since among the three methods is the only one that does not require solving an optimization problem during inference. 
However, the greatest advantage of \kenn\ over other architectures is its scalability. This is confirmed by the comparison of the execution times of the three methods: we found \kenn\ to be very fast as compared to the other two methods with an average of 7.96s required for a single run, as compared to the NN which requires 2.46s (on average of 1.83 seconds for each KE layer). A run of SBR cost 87.36s (almost 11 times slower than \kenn), while RNM required 215.69s per run (27 times slower)~\footnote{All the experiments have been run on the same architecture, an NVIDIA Tesla v100}.}





% \todo{\\
%     - kenn va meglio quando i dati scarseggiano\\
%     - anche per gli altri metodi, transductive meglio di inductive\\
% }


% Indeed, in \kenn\ the relations are considered only on the level of the KE. This is true also for RNM and SBR. 


% As mentioned previously, the three methods seem to have similar behaviors. In particular, we can not see anymore the large difference between KENN/RNM and SBR. 

% (Dire che caso transductive e weakly supervised, e li metodi come SBR funzionano meglio)

 

% \todo{appendix...}}

% By looking at Table~\ref{tab:comparison} we can notice that, differently from the inductive case, the three methods have similar effects on the accuracies, with the only exception of the 10\% split of the data, where KENN produces a much higher improvement over the NN and the 90\% case \todo{...}. 

% Notice that, although the final results are calculated as the mean of multiple runs, there are still some fluctuations and it is not possible to perfectly replicate the results obtained by~\cite{RNM} for the NN. For this reason, in Table~\ref{inductive_results} the NN has two columns, one with the results reported in~\cite{RNM}, another with the results obtained in our experiments. Since the results of the NN are slightly different in these two cases, the considered metric for the three methods is the improvement over the NN accuracy.


% \begin{table}
%     \caption{Results in terms of accuracy on the inductive variant of the task, ordered by the percentage of data used for training. The first three columns contains the results reported in~\protect\cite{RNM}.}
%     % , while my results are in the last three. Notice that the NN results are slightly different in the two versions}
%     \centering
%     \begin{tabular}{c|lll|lll}
%         \% Tr & NN & SBR & RNM & NN & \kenn\\
%         \hline
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         10 & 0.645 & 0.650 & {\bfseries 0.685} & 0.544 & 0.601 \\
%         &&  (+0.005) & (+0.040) && {\bfseries (+0.048)} \\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         25 & 0.674 & 0.682 & {\bfseries 0.709} & 0.629 & 0.671 \\
%         &&  (+0.008) & (+0.035) && {\bfseries (+0.041)}\\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         50 & 0.707 & 0.712 & {\bfseries 0.726} & 0.680 & 0.714 \\
%         &&  (+0.005) & (+0.019) && {\bfseries (+0.034)} \\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         75 & 0.717 & 0.719 & 0.726 & 0.733 & {\bfseries 0.754} \\
%         &&  (+0.002) & (+0.009) && {\bfseries (+0.021)} \\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         90 & 0.723 & 0.726 & 0.732 & 0.759 & {\bfseries 0.768} \\
%         &&  (+0.003) & (+0.009) && {\bfseries (+0.010)} \\
%         \hline
%         \hline
%     \end{tabular}
%     \label{inductive_results}
% \end{table}






% \todo{
% A bar plot of the results Figure~\ref{fig:comparison} shows the different accuracies improvements produced by the three methods at varying percentages of training data. (appendix plot) }

% Notice that, since we don't have all the data of the RNM and SBR experiments, it is not possible to provide the same analysis also for these methods. Indeed, to calculate p-values and confidence intervals the standard deviation is required.
%  For this reason, while 
%  \todo{we can be fairly confident about the ability of KENN to incorporate the knowledge into the NN
% %  , the comparison with the other two methods is not as statistically relevant. Additionally, since the number of runs performed in those experiments are only ten for each percentage of training data (as opposed to 500 of the KENN experiments), we could expect much bigger confidence intervals for SBR and RNM improvements. 
% %  However,
% we believe that this comparison can
% % still 
% provide us some useful information, in particular when comparing SBR with KENN and RNM.}
%  Indeed, the difference between SBR and the other two methods seems too large to depend only on the random choice of the nodes in the Training Set.




% An interesting \TODO{aspect of these results is that both KENN and RNM perform better than SBR. Notice that the first two methods are based on structure} while SBR injects the logic following \TODO{the regularization approach (see ... for a definition ...). Together with the experiments on VRD (see ...), where KENN outperformed LTN, these results give us additional ... of model approaches against loss methods.
% }.



% \todo{converging to similar results when the percentage of training is 90\%.}









% More on the distributions of the results over the 500 runs is available on Appendix~\ref{ap:inductive}.


% \TODO{Finally, Figure~\ref{fig:inductive_histograms} shows the distribution of the accuracies achieved by the NN and KENN (on the left side) as well as the distribution of the imporvements obtained by the injection of the logical rules (on the right). Based on these plots, we assumed these distributions to be normal, and we calculated the p-values for each training dimension. Since the number of runs, as well as the obtained improvements, are quite high, the resulting p-values are always close to zero.} More in details, the p-values are all in the range from 6.6e-183 (for 25\% of the training data) to 2.9e-09 (in the case of 90\%). For this reason we can safely reject the null Hypothesis. In other words, we are very confident that the improvements given by KENN do not depend on the random \TODO{ choices of the splits of the dataset.}


% \subsection{Results on transductive learning}

% \label{sec:results_collective_transductive}
% Table~\ref{transductive_results} shows the results of the various models on the transductive learning task. 


% \begin{table}[H]
%     \caption{Results in terms of accuracy on the transductive variant of the task. \todo{ridurre dimensioni.. solo delta (vorrebbe dire eliminare colonne NN (e anche descrizione ...) e rimuovere una riga per ogni percentuale)? Se facciamo cosi, possiamo avere una tabella singola per inductive e transductive}}
%     % , while my results are in the last three. Notice that the NN results are slightly different in the two versions}
%     \centering
%     \begin{tabular}{c|lll|lll}
%         \% Tr & NN & SBR & RNM & NN & \kenn \\
%         \hline
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         10 & 0.640 & 0.703 & {\bfseries 0.708} & 0.544 & 0.652\\
%         &&  (+0.063) & (+0.068) && {\bfseries (+0.108)}\\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         25 & 0.667 & 0.729 & {\bfseries 0.735} & 0.629 & 0.702 \\
%         &&  (+0.062) & (+0.068) && {\bfseries (+0.073)} \\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         50 & 0.695 & 0.747 & {\bfseries 0.753} & 0.680 & 0.744 \\
%         &&  (+0.052) & +0.058) && {\bfseries (+0.065)} \\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         75 & 0.708 & 0.764 & 0.766 & 0.733 & {\bfseries 0.788}\\
%         &&  (+0.056) & {\bfseries (+0.058)} && (+0.055)\\
%         \rule{0pt}{3ex}\hspace{-0.12cm}
%         90 & 0.726 & 0.780 & 0.780 & 0.759 & {\bfseries 0.808}\\
%         &&  {\bfseries (+0.054)} & {\bfseries (+0.054)} && (+0.049)\\
%         \hline
%         \hline
%     \end{tabular}
%     \label{transductive_results}
% \end{table}


% Note that, as mentioned previously, the results of the NN provided by~\cite{RNM} are similar to the case of inductive learning. In our case the results are identical. This is because the seed was chosen to be the same in both inductive and transductive learning. This allow us to have an even better comparison of the behaviours of KENN in inductive and transductive learning. Indeed, while the neural network predictions are exactly the same in the two cases, the improvements obtained by adding the knowledge (in all three methods) are much higher when using the citations between training and test nodes.




% Notice however that such improvement could depend on the much smaller accuracies produces by the NN of our experiments as opposed to the one obtained by~\cite{RNM}.

% \begin{figure}
%     \centering
%     % \makebox[\textwidth/2][c]{
%     \includegraphics[scale=0.4]{plots/transductive_learning_comparison.png}
%     % }
%     \caption{Comparison between KENN, SBR and RNM in terms of improvements over the NN on transductive learning. Black lines represent 95\% confidence intervals}
%     \label{fig:transductive_comparison}
% \end{figure}


% By looking at the confidence intervals, and considering that SBR and RNM's resuts are based on 10 iterations, we can not come to meaningfull conclusions on the comparison of the three methods. However, 
% as before, we can safely conclude that KENN is sensibly improving the performances of the NN (again, the p-values obtained are close to zero, and the confidence intervals are even smaller than the ones in the inductive case). }
% This can be also noticed from the histograms in Appendix~\ref{ap:transductive}, where the difference between the distribution of results of KENN and the NN can easily be seen with naked eyes.


% \begin{figure*}
%     \makebox[\textwidth][c]{
%         \includegraphics[scale=0.55]{plots/histograms_transductive.png}
%     }
%     \caption{Left: distributions of accuracies of the NN and KENN on 500 runs of Transductive Learning; Right: distributions of the improvements in accuracy produced by the KE.}
%     \label{fig:transductive_histograms}
% \end{figure*}

% \todo{(rimuovere, semplicemente citare lavori precedenti che mostrano che metodi basati su loss funzionano bene in contesti weekly supervised) To explain this behavior, we can reason about the properties of transductive learning, where all the methods have at their own disposal information about relations between training and test nodes. Like for inductive learning, the loss is calculated from the predictions on the training set nodes. However, if clause weights are high enough, the loss depends indirectly also on the values of the test nodes.
% To explain this property, lets look at Figure~\ref{fig:bias_kenn}. White nodes represent nodes of the test set. Suppose color red represents the class AI and blue ML. The value of the loss function does not depend directly on the value of node 9, since it is not in the training set. However, if the clause weight $w_{AI}$ of clause $c_{AI}: \lnot AI(x) \lor \lnot Cite(x,y) \lor AI(y)$ is high, then setting node 9 to class AI would influence node 3 prediction as well, pushing it towards the same prediction (AI). 
% % On the contrary, if we classify node 9 with the class ML, then node 3 could also be classified as ML.

% \begin{figure}
% 	\centering
% 	\input{tikz/transductive_propagation.tex}
%     \caption{\todo{An extreme example of a graph in a transductive learning scenario: the white nodes are available during training, but not their classes. }\todo{togliere!}}
%     % In this simple scenario, it is easy for the learning algorithm to make \kenn\ fit the data by forcing the satisfaction of the constraints and by classifying the test set nodes accordingly.}
%     \label{fig:bias_kenn}
% \end{figure}

% Summarizing, in the simple scenario of Figure \ref{fig:bias_kenn}, it is convenient for the model to predict nodes 9 and 8 as AI and ML respectively, forcing also the training nodes to be correctly classified. As a consequence, the loss is reduced and this kind of solution is rewarded by the training process. In this case, the KE produces a sort of regularization similar to the one of LTN and SBR., since it rewards solutions that make the constraints satisfied. }

% \section{\TODO{togliere...?} Clauses weights learning}
% \label{sec:scatter}

% We analyzed the efficacy of \kenn\ on learning the clause weights by analyzing their values after training and comparing them with the level of satisfaction of the constraints on the training data. 
% % More in details, we define the compliance of the training set with the constraints by \TODO{...}
% More in details, given a specific topic $k$\footnote{To simplify the notation, here we represent the topics as integers} and the corresponding clause ($\lnot k(x) \lor \lnot Cite(x,y) \lor k(y)$), we define the compliance of the Training Set with the constraint as the fraction of time in which papers of topic $k$ are cited by papers that are also of that topic.

% More in details, lets define $G = (V, E, T)$ as the graph containing the ground truth labels of the training set. Here $V$ is the set of nodes (papers), $E$ the sets of edges (citations), and $T: V \to [1,k]$ a function that maps each paper to the correct topic. Given a topic $k$, we define the clause compliance of $k$ as:
% $$
% C(G, k) = \frac{\sum_{v \in T_k} \sum_{u \in \mathcal{N}(v)} \mathbf{1}(u \in T_k)}
% {\sum_{v \in T_k} |\mathcal{N}(v)|}
% $$
% where $T_k = \{ v | v \in V \land T(v) = k \}$ is the set of nodes of topic $k$, $\mathcal{N}(v)$ is the function that returns the neighbours of node $v \in V$ and $\mathbf{1}(u \in T_k)$ is 1 if $u \in T_k$, 0 otherwise.

% Figure~\ref{fig:scatter_plot} shows a series of scatter plots (one for each percentage of training data) representing the correlation between learned clause weights and training data compliance with the clauses. Each point corresponds to a topic in a specific run and its coordinates are given by the compliance value for the topic ($y$ axis) and the learned clause weight ($x$ axis). In total there are 3000 points, each of which corresponds to a specific topic and run in the inductive learning scenario.

% The plots suggest a correlation between the two values, in particular with high percentages of training data. This means that, in this specific dataset, \kenn\ seems to be capable of learning the clause weights from the data at its disposal. 

%     Moreover, we can notice an increase in variance when the constraints are only partially satisfied. For instance, the constraint applied on topic AI is in general satisfied half of the times and the values of the corresponding clause weight is more sparse as compared with other topics. This behaviour could be explained by the random initialization of the NN parameters since the impact of a clause depends on the initial predictions of the NN. Indeed, as seen in Section~\ref{preact}, the knowledge is added at the level of the preactivations and it could produce bigger changes when the preactivations are close to zero (see Figure~\ref{fig:logistic} for more details). 

%     This means that the CE produces different degree of changes to each node, and the random initialization of the NN affects the choice of which nodes receive higher modifications. If the ones that are highly modified by the CE correspond to the nodes for which the constraints is satisfied, then the impact of the CE on the final prediction is positive. On the contrary, if the CE produce small changes when the constraint is satisifed, and big changes when it is not, then the CE produces a degradation of the performances and the corresponding clause weight is reduced. In other words, when the constraint is only partially satisfied, the effect of the associated CE is more randomic and, as a consequence, the clause weight distribution is more sparse.


\section{Conclusions}
\kenn\ is a NeSy architecture that injects prior logical knowledge inside a neural network by stacking a residual layer on its top.
%  increase the satisfaction of a set of clauses on the predictions of a NN by stacking a residual layer on top of the model.
In~\cite{kenn}, it proved to be able to effectively inject knowledge in the context of multi-label classification tasks. In this work, we extended \kenn\ for relational domains, where the presence of both unary and binary predicates doesn't allow for the usage of the simple tabular representation of the data used in the previous version of the framework. \new{Moreover, we propose a strategy to deal with the violation of the independence assumption made by \kenn.} The experiments on Citeseer show \new{the effectiveness of this strategy, obtaining} statistically relevant improvements over the NN performances, meaning that \kenn\ can successfully inject knowledge even in the presence of relational data. Finally, \kenn\ provided quality results also in comparison with other two NeSy frameworks. In particular, the large difference in performances between \kenn/RNM and SBR provides additional evidence in support of model-based approaches in comparison to regularization ones\new{, with \kenn\ the best option in terms of scalability.}
%  \TODO{Indeed, in previous experiments, \kenn\ showed already better performances in comparison with LTN, another regularization approach.}




% \section*{Acknowledgements}
% We would like to thank Riccardo Mazzieri for his help on conducting the experiments on Citeseer. Many thanks also to Artur d'Avila Garcez, Alessandro Sperduti, Marco Gori, Sagar Malhotra and Tommaso Carraro for useful suggestions and feedbacks.

% \section*{Funding}
% This work has been partially supported by the EU H2020-ICT-2018-2 RIA project AI4EU  (grant agreement 825619).






% If the nodes with higher changes are the one for which the constraint is satisfied, then the impact of the KE on the final predictions is positive and the clause weight tends to increase. On the contrary, if the KE produces small changes for nodes 

% This means that the KE produces different degree of changes based on the random initialization of the NN and adding the knowledge could be beneficial or not depending on such initialization. Indeed, if the confidence of the NN is high for the nodes that do not satisfy the constraint, and low otherwise, then the impact of the KE on the final predictions is positive and the clause weight tends to increase. 

% If the NN returns high level of confidence for the samples when the clause is not satisfied, then the negative impact that comes by enforcing the clause will be low.


% \begin{figure*}
%     \makebox[\textwidth][c]{
%         \includegraphics[scale=0.45]{plots/corrplots.png}
%     }
%     \caption{Correlation between learned clause weights and clauses satisfaction on Training Set for the five percentages of training data}
%     \label{fig:scatter_plot}
% \end{figure*}

% More precisely, it enforces the satisfaction of the constraints like SBR and LTN do.




% This can be explained by the fact that in transductive learning \kenn\ works differently than the usual. More precisely, it enforces the satisfaction of the constraints like SBR and LTN do. To explain this property, lets look at Figure~\ref{fig:bias_kenn}. 
% % For simplicity of exposition, the picture shows a really extreme example where the training graph is disconnected. However, the property holds in general, particularly when the amount of test nodes 
% As before, white nodes represent nodes of the Test Set. \kenn\ can easily fit the data just by setting the values accordingly with the knowledge. For example, lets say that color red represents the class AI. The value of the loss function does not depend directly on the value of node 9, since it is not in the Training Set. On the contrary, the prediction for node 3 depends on such value if the clause weight $w_{AI}$ of clause $c_{AI}: \forall x \ \forall y \ AI(x) \land Cite(x,y) \to AI(y)$ is high. In such a case, a classification of node 9 as AI would determine 3 to be classified as AI as well. Therefore, it is convenient for the model to learn a high value for $w_{AI}$ and predict node 9 as AI, since this will force also 3 to be AI and as a consequence the Loss would be reduced. In this case, the KE produces a sort of regularization similar to the one of LTN and SBR, since it rewards solutions that makes the constraints satisfied. 

% \TODO{This property holds particularly when there are many nodes in the Test Set, since its through them that \kenn\ enforce the satisfaction of the constraints.}

% Notice that t

% therefore, to make correct the predictions of nodes 1 and 2 (reducing the loss), it is convenient for \kenn\ to set the values of nodes 3 and 4 accordingly to the knowledge, meaning that \kenn\ in this case tend to force the satisfaction of the clauses.

% Finally, the picture shows a really extreme example where the training graph is disconnected. Notice that this was just for simplicity of exposition, and in general 




% \begin{figure*}
%     \makebox[\textwidth][c]{
%         \includegraphics[scale=0.55]{Figures/bias_kenn.png}
%     }
% \end{figure*}


==> Relational KENN/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


In the last decade, deep learning approaches gained a lot of interest in the AI community, becoming the state of the art on many fields, such as Computer Vision~\cite{image_classification}, Machine Translation~\cite{machine_translation}, Speech Recognition~\cite{speech_recognition}, etc. 
% However, the main downside of such methods is that they are demanding in terms of training data.
\new{
Indeed, Neural networks (NNs) are suited for pattern recognition, even in the presence of noisy data. They are particularly good at mapping low-level perceptions to more abstract concepts (for instance, going from images to classes). However, it is hard for a NN to reason with these high-level abstractions. Furthermore, NNs are demanding in terms of training data. On the other hand, pure logical approaches are not suited for learning from low-level features and they struggle in the presence of noise. Nevertheless, they perform well in reasoning with highly abstract concepts and learning from a small number of samples. Given these opposite strengths and weaknesses, it is not a surprise that a lot of interest has been drawn toward Neural-Symbolic (NeSy) systems. Indeed, the goal is to combine these two paradigms to obtain the best of the two worlds.}

% \todo{(rimuovere? e sostituire)
% On the other hand, human beings are capable of learning new concepts with few examples (Few Shot Learning) and even in some cases with zero experience (Zero-Shot Learning). One of the main reasons is due to their ability to make use of previously acquired knowledge. 
% While in the case of humans such knowledge is often in the form of natural language definitions, Neural-Symbolic Integration (NeSy) methods are focused on knowledge expressed in terms of a set of logical formulas.}

\new{Among NeSy methods} there is \kenn\ (\emph{Knowledge Enhanced Neural Network})~\cite{kenn}, \new{a model composed of a Neural Network enhanced with additional layers which codify logical knowledge.} \kenn\ has multiple advantages over other NeSy methods, such as its capacity to learn \emph{clause weights} and the ability to impose the knowledge not only during training but even at inference time.
In particular, \kenn\ showed remarkable results on the Predicate Detection task of Visual Relationship Detection Dataset (VRD Dataset)~\cite{visual2} using a manually curated prior knowledge proposed by~\cite{IvanThesis}, outperforming the previous state of the art results, with really good performances on the \emph{Zero Shot Learning} sub-task~\cite{kenn}. Moreover, it outperformed Logic Tensor Networks~\cite{LTN}, one of its major competitors, using the same knowledge.

Despite its good empirical results, \kenn \ has been applied only on multi-label classification tasks with no relational data. Indeed, a limitation of \kenn\ resides in its inability to take into account binary predicates. This is because \kenn \ expects the NN's predictions to be stored in a matrix format, where the columns represent different unary predicates and the rows their possible groundings (i.e., substitutions of the free variable for such predicates). 
% \TODO{KENN works with batches of data in matrix form, where each column represents a unary predicate. For this reason, it is not straightforward to apply KENN on relational data, where binary predicates are available as well.}
For this reason, 
% \kenn \ is suited for multi-label classification problems, and 
it is not straightforward to apply \kenn\ to relational data, where binary predicates are available.

% While multi-label classification is an important topic in machine learning, the usage of knowledge is particularly relevant in the context of relational domains.
% Statistical Relational Learning (SRL)~\cite{SRL}.
% For this reason, 
In this paper,
we propose an updated version of \kenn\ which can deal with relational data.
% these kinds of domains. 
\new{Particular attention was paid to defining a scalable strategy to deal with binary predicates, obtaining good performances in terms of execution time. Indeed, \kenn\ assumes independence between the logical rules, allowing for scalable inclusion of the underlying knowledge. However, the assumption is often violated in real scenarios, in particular in the contexts of relational domains. To deal with this problem, we propose a strategy that consists of adding multiple logical layers inside the model. We provide proof of the efficacy of this strategy in a simple scenario with two logical rules. Additionally, we tested this idea on Citeseer, a dataset for Collective Classification~\cite{collective_classification}, showing that the additional layers improve the performance of the model.
%  even in more complex scenarios.
Moreover, 
}
% \todo{In building this extension, we pay particular attention to scalability, since ... }
% \todo{(rimuovere???)
% Additionally, the usage of knowledge can help to represent relational data inside a neural network, which is not a straightforward task since neural networks' inputs are represented using tabular data (they can be vectors, matrices, or in general tensors)~\cite{NN_relational}.}
% \todo{aggiungere qualcosa sui vari layers}
% \todo{Moreover, we provide new experiments to test the effectiveness of \kenn\ in these types of contexts. For this purpose, we applied \kenn\ on Citeseer~\cite{citeseer}, a standard dataset for Collective Classification~\cite{collective_classification}.} T
the experiments on this dataset 
% are particularly relevant since they 
provide
% insight into the usage of \kenn\ on relational domains and they give us 
a comparison between \kenn\ and two other approaches: Semantic Based Regularization (SBR)~\cite{SBR} and Relational Neural Machines (RNM)~\cite{RNM}. 
% The evaluation was conducted with two different learning paradigms of Collective Classification, namely inductive and transductive learning. 
% Moreover, the \new{three methods have been} applied to different splits of the dataset to evaluate \new{their} performances at varying numbers of training samples.



% which can be seen as constraints on the possibile outcomes of a classifier.

% The ability to exploit provided knowledge is crucial for effectively learn new concepts when training data is scarce. Among the methods for combining neural networks models and logical knowledge

% \TODO{(Rimuovere)

% Such knowledge could come for experience on different tasks. For instance, when learning to move around and avoid obstacles, humans can effectively learn the three-dimensional structure of the world by constructing an internal representation of it. When approaching a new task where visual data must be processed, they can make use of the previously learned representation, transferring the acquired knowledge into a new domain.

% Another type of knowledge is the one provided by other human beings. For example, suppose we tell a kid: ``A unicorn is a horse with a horn in its forehead''. Although the kid has no previous experience of unicorns, he will be able to recognize them, for example when watching a movie. This ability to exploit provided knowledge is crucial for effectively learn new concepts when training data is scarce.
% }



% \TODO{ (cambiare un po' e introdurre KENN, parlare dei vantaggi di KENN e collegarsi ai risultati ottenuti in precedenza.. da li si va direttamente alle modifiche apportate)  



% In this paper, we are going to focus on this second type of knowledge. 
% While in the case of humans such knowledge is often in the form of natural language definitions, here it is provided as a set of logical formulas. }






%ince both base NN and KE are differentiable, the entire architecture is differentiable end-to-end, making it possible to apply % back-propagation algorithm on the whole model.

% The KE changes the values of the predictions $\by$ of the base NN into $\by'$ in order to increase the truth value of each clause $c \in \clauses$. This is achieved by calculating, for each clause $c \in \clauses$, a different modification of the $\by$ vector which increases the satisfaction of $c$. The final predictions $\by'$ are obtained by adding to the base NN's outputs $\by$ the weighted sum of such changes using as weights parameters $w_c$.

% For each clause $c \in \clauses$, KE internally produces the change to be applied to the predictions $\by$ in order to increase $c$ satisfaction.

% It then calculates the final predictions $\by'$ by adding to the NN outputs the weighted sum of such changes using as weights parameters $w_c$.


% While in literature many methods already exist, no consensus over a general solution has been reached yet. Moreover, among the existing methods, few recent works have been done on the injection of the logic directly into the structure of the model. On the contrary, a prominent line of research is based on the idea of enforcing the knowledge at the level of Loss function by optimizing during learning the satisfaction of the logical rules.

% \TODO{
% Great attention was put also on scalability, particularly in the context of relational domains. The objective was to build a model that englobe the knowledge in its structure and that is fully differentiable, making it trainable end to end.  Scalability is not the only advantage of this type of approach. Indeed, by including the knowledge into the model, the weights of the rules do not have to be known a priori.}


% An important question arises: what does it mean to increase the satisfaction of a clause? We use fuzzy semantic \ls{AGGIUNGI CITAXIONE A FUZZY LOIGC BOOK}, where the satisfaction of a clause is given by applying a t-conorm function $\bot$ on the truth values of the literals of the clause. Therefore, the objective of the final layer should be increasing the value of the chosen t-conorm.
% \ls{LA FRASE SEGUENTE IO NON LA CAPISCO} However, we are not relying on an optimization process to add knowledge, so it is not possible to just optimize the value of the t-conorm at run time. On the contrary, we want to inject the knowledge as a differentiable layer on top of a neural network: the optimization must be done analytically!


% \TODO{
% , given a disjunction of $n$ literals, and  the truth values of such literals, it returns a vector $\delta \in [0,1]^n$ such that

% While fuzzy logic has the goal to define an interpretation of ... with truth values in the range $[0,1]$, in this case the goal is to define a function that given an initial interpretation, returns an enhanced intepretation that }

% I divided the development of \kenn\ into two different sub-tasks: the first one was the task of developing a method for the injection the knowledge, while the second 



% In the first stage of development, the focus was on the injection of knowledge composed of FOL clauses with only one free variable. This can be useful in the context of multi-label classification.

% In a second stage, I extended the types of accepted rules with FOL clauses with a higher number of variables, moving from multi-label classification to SRL tasks. The major challenge in this second stage was to keep the model scalable while working with graphs. To solve the problem, I proposed a solution that consists on implementing a Relational Database using TensorFlow and developing a differentiable version of queries on this database. While this solution was only applied in the context of \kenn, in future work it can be extended to a more general case, where differentiable queries could be used to generate new Neural Network architectures that can work with relational domains.

% in the second one the interest was on 

% in the first one the injected knowledge is composed of FOL clauses with only one free variable which can be useful in the context of multi-label classification. 

% A second objective was to expand the types of accepted rules with FOL clauses with higher number of variables, moving from multi-label classification to SRL tasks. \TODO{qui collegarsi a DB relazionali}


% \TODO{In our previous work~\cite{kenn}, we tested \kenn\ on 

% % In a second experiment, we tested \kenn\ on 
% the Predicate Detection} task of Visual Relationship Detection Dataset (VRD Dataset)~\cite{visual2} using a manually curated prior knowledge proposed by~\cite{IvanThesis}, outperforming previous state of the art results, with really good performances on the \emph{Zero Shot Learning} sub-task.
% % The task consists in finding the relationships between pairs of objects inside an image and it contains a \emph{Zero Shot Learning} sub-tasks where the objective is to predict types of relationships not available at training time. In this dataset, \kenn\ outperformed state of the art methods, with the best results on \emph{Zero Shot Learning}. 
% % This experiment confirms the fact that background knowledge plays a key role in machine learning when training data is scarce. 
% Moreover, \kenn\ outperformed Logic Tensor Networks, one of its major competitors, using the same knowledge.

% However, notice that previous experimets have been applied only on multilabel classification problems with no relational data. Here we provide new experiments applied to test the efficacy of \kenn\ even in the context of relational domains. For this purpose, we applied \kenn\ on Citeseer~\cite{citeseer}, a standard dataset for Collective Classification~\cite{collective_classification}. The experiments on this dataset are particularly relevant since they provide some insight on the usage of \kenn\ on relational domains and they give us a comparison between \kenn\ and two other approaches: Semantic Based Regularization (SBR)~\cite{SBR} and Relational Neural Machines (RNM)~\cite{RNM}. The evaluation was conducted with two different learning paradigms of Collective Classification, namely Inductive and Transductive Learning. Moreover, the experiments were applied to different splits of the dataset to evaluate the three methods performances at the varying of the number of training samples.

% % The paper is divided as follows: Section~\ref{ch:rel_works} presents the state of the art. In Chapter~\ref{ch:kenn} we introduce the theory behind \kenn. Chapter~\ref{ch:architecture} defines the architecture of the model, with a particular focus on relational domains. The related work is presented in Chapter~\ref{ch:rel_work_2} together with a comparison with \kenn.
% % % \ with other prominent methods in the literature.
% % In Chapter~\ref{ch:implementation} the implementation details are highlighted. Chapters~\ref{ch:multilabel} and~\ref{ch:collective} present the experiments on multi-label and Collective Classification, respectively. Finally, Chapter~\ref{ch:conclusions} provides the conclusions and the future work.

% % The final results are in line with state of the art methods. More importantly, the obtained results shows that even for relational data, with a minimal required effort, \kenn \ is capable of increasing the performances of the NN is applied to.

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "paper KENN"
% %%% End:


==> Relational KENN/kenn.tex <==


\section{Knowledge Enhanced Neural Networks}
% As previously mentioned, \kenn\ is a method for knowledge injection inside neural networks models. 
% Before diving into \kenn\ architecture, lets define the language used to represent the prior knowledge\:
% \subsection{Prior knowledge}
% \label{sec:prior_knowledge}
We define the prior knowledge in terms of formulas of a function-free first order language $\L$. Its signature is defined with a set of domain constants $\C \triangleq \{a_1, a_2, ... a_m \}$
% \TODO{uso gia $l$ da qualche parte? controllare} 
and a set of predicates $\P \triangleq \{P_1, P_2 ... P_q \}$.
% For each predicate $P_i$ we denote its arity with $n_i$.
In our setting, predicates can be unary or binary/
% ~\footnote{\todo{dire che il metodo puo essere esteso a altre arieta??}}. Unary predicates can be used to express properties of singular objects. For instance, to represents that a person $a \in \C$ is a smoker, we can use $Smoker(a)$, where $Smoker \in \P$.
%  is a predicate with arity one. 
Binary predicates can express relations among pairs of objects in the domain, e.g. $Friends(a,b)$ states that person $a$ is a friend of $b$.
% ~\footnote{Predicates with arity greater than two are not considered in this work}.
The prior knowledge is defined as a set of clauses: $\clauses \triangleq \{ c_1, c_2, ... c_r \} $. A clause is a disjunction of literals, each of which is a possibly negated atom:
	$
	c \triangleq \bigvee\limits_{i=1}^{k} l_i
	$, where $k$ is the number of literals in $c$ and $l_i$ is the $i^{th}$ literal. We assume that there are no repeated literals.
% A literal is a predicate \TODO{, which is defined as $P(x)$ or $R(x,y)$, where $P$ and $R$ are unary and binary predicates respectively, and $x$ and $y$ are the two variables. }
Since we are interested in representing only general knowledge, the literals do not contain any constant, only variables that are assumed to be universally quantified. If the predicate is binary, the two variables are $x$ and $y$, otherwise only $x$.
% only the variables $x$ and possibly $y$ (if the predicate is binary, it contains both, otherwise only $x$). Such are assumed to be universally quantified. 
When an entire clause contains only variable $x$ (i.e., only unary predicates), we call it \emph{unary}. Similarly, if it contains both $x$ and $y$ we call it \emph{binary}\footnote{We restrict to the case where clauses contain at most two variables}.

% \TODO{Notice that the previous clause has no constants and the two variables $x$ and $y$ in it are assumed to be universally quantified. This is because we are interested in representing general knowledge, and in the following, we will always apply this assumption implicitly to each clause in our knowledge.}

As an example, the clause $\lnot Smoker(x) \lor Cancer(x)$ is unary and states that all smokers have also cancer (notice that the clauses are not assumed to be hard constraints). Instead, the clause
\begin{equation}
	\lnot Smoker(x) \lor \lnot Friends(x,y) \lor Smoker(y)
	\label{eq:clause}	
\end{equation}
is binary. It states that if a person $x$ is a smoker and he is a friend of another person $y$, then $y$ is also a smoker. We will use extensively this clause in the remaining of the paper, referring to it as $c_{SF}$.

%  Notice that $\clauses$ is used to represent general knowledge, which means that each atom inside a clause does not contain any constant and the clause is assumed to be universally quantified.

We define the grounding of a unary clause $c$, denoted by $c[a]$, as the clause obtained by substituting the $x$ variable with constant $a$. Similarly, if $c$ is binary, its grounding $c[a,b]$ is obtained by substituting $x$ and $y$ with $a$ and $b$ respectively. For instance, 
% given two specific persons $a$ and $b$, 
the grounding $c_{SF}[a,b]$ of the clause defined in~ Eq.\ref{eq:clause} correspond to
$
\lnot Smoker(a) \lor \lnot Friends(a,b) \lor Smoker(b)
$.
% We will denote with $\clauses[\C]$ the set of all the grounded clauses.

\subsection{\kenn\ architecture}
Suppose we have a NN for a classification task which takes as input a matrix $\bx \in \Reals^{d \times n}$ containing $n$ features for $d$ samples, and returns an output $\by \in [0,1]^{d \times q}$ which contains the predictions for $q$ classes corresponding to the $q$ predicates.
A prior knowledge $\clauses$ is also provided. 
% However, differently from the Section~\ref{sec:prior_knowledge}, in \kenn\ only unary clauses are allowed (see Section~\ref{sec:rel_kenn} for the extension to binary clauses). The knowledge 
It can be used by \kenn\ to improve the predictions of the NN. 
% For instance, the clause $\forall x \ (\lnot Smoker(x) \lor Cancer(x))$ can be used by \kenn, in conjunction with the NN, to predict the two labels $Smoker$ and $Cancer$.

% The logical rule assumed to be universally quantified.

% \kenn\ enhances the NN's prediction by injecting the background knowledge in an additional final layer. This layer, called \emph{Knowledge Enhancer} (KE), is designed to increase the satisfaction of the clauses by modifying the initial predictions made by the NN.
Figure~\ref{fig:KENN_overview}(left) shows a high-level overview of \kenn \ \new{where} a residual layer, called \emph{Knowledge Enhancer} (KE), is inserted between the NN and the final activation function. The role of KE is to revise the final predictions returned by the NN in order to increase the truth value of each clause $c \in \clauses$. It does so by calculating a residue $\bdelta$, a matrix that is added to the predictions of the NN. 

\begin{figure}%[H]
	
	\centering
	% \makebox[\textwidth][l]{
        \includegraphics[scale=0.16]{imgs/KENN_overview.png}
    % }
	\caption{Model architecture. Left: \kenn\ model overview. 
	% Knowledge Enhancer (KE) receives in input $\bz$, the pre-activations of the NN's predictions. It returns the residual matrix $\bdelta$ which is added to $\bz$ to increase the satisfaction of the prior knowledge $\clauses$ in the final output $\by$. 
	Right: Knowledge Enhancer.
	% For each clause $c_i \in \clauses$, it calls a CE which returns the residue $\bdelta_i$ for $c_i$. The $\bdelta_i$ are then multiplied by the corresponding clause weights $w_i$ and summed up to obtain the final $\bdelta$ matrix.
	% features are given as input to a neural network (NN) and predictions on predicates values are returned. Knowledge Enhancer modifies the predictions' pre-activations based on logical constraints ($\clauses$). After this process, the activation function is called.
	}
	\label{fig:KENN_overview}
\end{figure}


% On this behalf, 

% Our goal is to create a method for injecting logical prior knowledge into a neural network model, so it can learn more efficiently new concepts by mixing learning capabilities with logical inference.
% \TODO{Similarly to human beings, the neural network should be able to take into account the knowledge and combine it with its learning abilities.}


% \kenn\ exploits prior knowledge about the domain of interest. Such knowledge is expressed by a set of logical rules. For instance, in an image classification task the rule $\forall x \ (Dog(x) \to Animal(x))$, stating that dogs are animals, can be used by \kenn\ to predict the two labels $Dog$ and $Animal$. In \kenn\ all the rules are represented as clauses, i.e. disjunctions of literals, and they are assumed to be universally quantified.

% Suppose we have a Neural Network (NN) for a classification task, which is called \emph{NN}, \kenn\ enhances its prediction by injecting the background knowledge in an additional final layer. This layer, called \emph{Knowledge Enhancer} (KE) is designed to increase the satisfaction of the clauses by modifying the NN's predictions.

% It is given a neural network, called \emph{NN}, that takes in input the feature vector $\bx \in \Reals^n$ of an object and returns an output $\by \in [0,1]^m$ which contains the predictions for $m$ classes. A background knowledge $\clauses$ is also provided and it represents constraints on the $m$ classes to be predicted.

% Predictions $\by$ are revised by a function, called \emph{Knowledge Enhancer} (KE), that force the satisfaction of the logical constraints in $\clauses$.
 

The KE works in the pre-activations space, i.e. on $\bz$, and the activation function ($\sigma$) is called later. In order for \kenn\ to work, the activation function must be monotonic and return values in the range $[0,1]$~\footnote{For more details on why the KE is applied on pre-activations, please refer to~\cite{kenn}}.
% In KENN, the predictions $\bz$ of the NN are revised by a residual layer, called \emph{Knowledge Enhancer} (KE), which updates $\bz$ into $\by'$ to increase the truth value of each clause $c \in \clauses$. 
Since both NN and KE are differentiable, the entire architecture is differentiable end-to-end, making it possible to apply back-propagation algorithm on the whole model. Figure~\ref{fig:KENN_overview}(right) shows the architecture of KE, which calculates the residual matrix $\bdelta$.

% \begin{figure}[H]
% 	\centering
% 	% \makebox[\textwidth][l]{
%         \includegraphics[scale=0.18]{imgs/KE.png}
%     % }
% 	\caption{Knowledge Enhancer architecture. For each clause $c_i \in \clauses$, it calls a CE which returns the residue $\bdelta_i$ for $c_i$. The $\bdelta_i$ are then multiplied by the corresponding clause weights $w_i$ and summed up to obtain the final $\bdelta$ matrix.}
% 	\label{fig:KE}
% \end{figure}

% \TODO{KE takes as input the matrix $\bz$ containing the pre-activations of the final predictions generated by the NN, and outputs the residual matrix $\delta$, which contains the changes to be summed to $\bz$ to increase the satisfaction of $\clauses$. It increases the satisfaction of each clause separately, obtaining $|\clauses|$ different matrices, each of which represents the changes to be applied on $\bz$ to improve the satisfaction of a specific clause $c$. }

More in details, for each clause $c\in\clauses$, the KE contains a submodule, the \emph{Clause Enhancer} (CE), which proposes the changes $\bdelta_c$ to be applied on the NN's preactivations in order to increase the satisfaction of $c$. Indeed, the CE computes a soft differentiable approximation of a function called \emph{t-conorm boost function} (TBF). Intuitively, a TBF is a function \mbox{$\phi: \Reals^k \to \Reals_+^k$} that proposes the changes to be applied on the pre-activations $\bz$ of $k$ truth values, such that $\bot(\sigma(\bz + \phi(\bz))) \geq \bot(\sigma(\bz))$, where $\bot: [0,1]^k \to [0,1]$ is a t-conorm function,
% ~\footnote{Notice that in literature a t-conorm is defined as a binary operator. W.l.o.g., due to associativity and commutativity, w}
used in fuzzy logic to represent the semantics of the disjunction operator~\footnote{In \cite{kenn}, function $\phi$ is called $\delta$. Here we changed the name to avoid confusions with its output which is also referred as $\delta$}. In~\cite{kenn} it has been defined the function 
\begin{equation}
	\phi(\bz)_i = 
	\left\{
	  \begin{array}{ll}
	1 \ \ \ & \mbox{if $i = \argmax_{j=1}^n z_j$} \\
	0 & \mbox{otherwise}
	\end{array}
	\right.
	\label{eq:phi}
\end{equation}
and proved that such a function is the optimal TBF for
%  a specific t-conorm, namely 
the G\"{o}del t-conorm. 
% As mentioned previously, 
\kenn\ employs the softmax function
as a continuous and differentiable approximation of $\phi$.
%  \new{which corresponds to the softmax function}, allowing the integration with neural networks.
 
The $\bdelta_c$ matrices are combined linearly inside the KE to obtain the final change $\bdelta$ to be applied on the NN's predictions, and finally the $\bdelta$ is summed to the initial pre-activations $\bz$ and passed to the activation function:

\begin{equation}
	\begin{split}
	y_{P(a)} &= \sigma \bigl(z_{P(a)} + \sum_{\substack{c \in \clauses\\ P(x) \in c}} w_c \cdot \delta_{c[a],P(a)}\bigr)
	\end{split}
	\label{eq:final_intepretation_unary}
\end{equation}

where $w_c$ is the \emph{clause weight}, $P(a)$ a grounded atom, $y_{P(a)}$ its final prediction, and $z_{P(a)}$ the NN's pre-activations. Finally, $\delta_{c[a],P(a)}$ is the change applied to $P(a)$ based on the grounded clause $c[a]$:
\begin{equation}
    \label{eq:deltac}
  \delta_{c[a],P(a)}=\begin{cases}
    \phi(\bz_c)_{P(a)} & \mbox{if $P(a)\in c[a]$} \\
    -\phi(\bz_c)_{\lnot P(a)} & \mbox{if $\neg {P(a)}\in c[a]$} 
	% \\
    % 0 & \mbox{Otherwise}
  \end{cases}
\end{equation}
where $\bz_c$ are the pre-activations of literals of $c$.
% Finally, $w_c$ is the \emph{clause weight}, a learnable parameter associated with clause $c$ which determines the strength of $c$, i.e., it defines the influence that the clause has on the final predictions.  
% Differently from other Neural-Symbolic integration approaches, clauses weights are not given, but they are learned. 
% Notice that, by assigning zero to clause weights, \kenn\ can learn to ignore clauses in the prior knowledge that are not fully satisfied inside training data.\todo{questa cosa e ripetuta molte volte e non fa parte dei contributi del paper.. tagliare un po' in giro (magari sull'abstract)}

\new{
Note that applying a linear combination of the $\bdelta_c$ matrices can be done under the assumption of independence between the clauses. 
% Although such an assumption is in general not correct, it allows for a much more scalable architecture. However,
When multiple clauses share common predicates
% , the assumption is violated. As a consequence, in such scenarios, 
the changes proposed by \kenn\ could only partially improve the satisfaction of the knowledge. We will further analyze this problem in Section~\ref{sec:reasoning}}.

% \TODO{In Section~\ref{sec:scatter} we will further analyze this ability of \kenn\ to learn the clause weights by inspecting their value after training.}

==> Relational KENN/relational.tex <==


\subsection{Extending \kenn\ for relational domains}
\label{sec:kenn_extension}

% \TODO{(eliminare o spostare dopo e modificare??)
% In many scenarios we want to use batches of data, which would require to modify the structure of the model graph for each batch, in particular after each training step, since the groundings are constantly changing and for each grounding a different CE is instantiated. Notice that, even if the CEs are different, the internal operations are the same and the only change is the provided input. For these reasons, we want to instantiate a single CE for each clause $c$ which works in a single batch containing all possible groundings of $c$.}

% \TODO{spostare prima la descrizione della matrice}

In the architecture defined so far, the groundings involve a single object and $\bz$ is defined as a matrix, where columns represent predicates and rows constants. Fig.~\ref{fig:z}(left) introduces 
% more in details 
the representation of $\bz$: it is defined as a matrix such that the element $z_{ij}$ contains the pre-activation of $P_j(a_i)$, with $P_j$ the $j^{th}$ predicate and $a_i$ the $i^{th}$ constant.

\begin{figure}
	\centering
	% \makebox[\textwidth][l]{
        \includegraphics[scale=0.13]{imgs/representation.png}
    % }
	\caption{The representation of NN's final pre-activations. Left: unary case. Right: representation of relational data. Pre-activations are represented as integers instead of reals to simplify the figure.}
	\label{fig:z}
\end{figure}

Note that this kind of representation is common when working with neural networks since the columns (predicates) correspond to the labels and the rows (groundings) to the samples. An important aspect of this representation lies in the fact that each grounded atom can be found in the matrix exactly one time. This allows to parallelize computations of Equation~\ref{eq:final_intepretation_unary} since a grounded clause involves only atoms in the same row, and each row can be managed in parallel inside a GPU. This can be done only if the same atom does not appear in multiple rows, since the changes are applied independently to each row and are not aggregated together. This property always holds with unary clauses.


% \subsubsection{Relational data representation \todo{togliere sotto sezioni in giro, titolo occupa molto spazio}}

% \label{sec:relational_representation}

To represent relational data, we extend \kenn\ with an extra matrix $\bz_B$, which contains the binary predicates' pre-activations. For uniformity of notation we use $\bz_U$ to denote the unary matrix $\bz$ of the not relational \kenn.
% contains as many rows as objects in the domain and as many columns as unary predicates. It is exactly the same as $\bz$ of Fig.~\ref{fig:z}(a).
Matrix $\bz_B$ contains one row for every pair of objects we are interested in and a column for each binary predicate. 
% However, this time the variables involved are two and the considered predicates are only binary.
% Notice that we might not want to include all the pairs of objects in $\B$, because the application of binary predicates of some pairs might be meaningless. For instance, as already mentioned, the $Friends$ predicate applied to $(a,a)$ is not interesting.
% $\B$ has one column for each binary predicate and other two columns $s^x$ and $s^y$ that indicate the first and the second component of the
% pair. In the relational database analogy they can be seen as foreign keys to table $\U$. As with $\U$, each row represents a different grounding of the predicates, with the difference that in this case the predicates are binary and the variables to be substituted are two. More precisely, $\B_{i,j}$ corresponds to the value of predicate $B_j$ for the substitution $(x / o_{s^x_i}, y / o_{s^y_i})$:
% $$\B_{i,j} = B_j(o_{s^x_i},o_{s^y_i})$$
% For instance, in Fig.~\ref{fig:representation}(b): $s^x_0 = 0$ and $s^y_0 = 1$, which means that row $0$ of matrix $\B$ is referring to the pair of objects $(o_0,o_1)$.
% \begin{figure}
% 	\centering
% 	% \makebox[\textwidth][l]{
%         \includegraphics[scale=0.1]{imgs/graph.png}
%     % }
% 	\caption{Representation of relational data in \kenn. Pre-activations are represented as integers instead of reals to simplify the figure.}
% 	\label{fig:graph}
% \end{figure}
Fig.~\ref{fig:z}(right) shows this representation using the classical Smoker-Friends-Cancer example, where the domain is composed of three constants (persons) $\C = \{a, b, c\}$, the unary predicates are $S$ and $C$ (for $Smoker$ and $Cancer$), and a binary predicate $F$ (for $Friends$). The blue box shows the graph representation with nodes and edges labelled with pre-activation of unary and binary predicates respectively. The grey box shows the corresponding matrix representation used by  \kenn. Notice that it is not required that the entire graph is computed by the NN. For instance, in the experiments on Citeseer, the $Cite$ predicate is provided directly as a feature (see Section~\ref{sec:collective}).



% \subsubsection{\kenn\ for relational domains - An overview}
% \subsubsection{Working with binary knowledge}
% \label{sec:rel_kenn}

% \TODO{immagine architettura}
% In \TODO{Fig.~\ref{fig:relational_kenn}(a)} t
The architecture of \kenn\ for relational domains is
%  introduced. This is 
very similar to the architecture of traditional \kenn\ of Fig.~\ref{fig:KENN_overview}, with KE substituted by a \emph{Relational KE} (RKE). From a high level perspective, the RKE differs from the traditional KE on the amount of inputs and outputs. As seen before, in the relational case the pre-activations are divided in two different matrices ($\bz_U$ and $\bz_B$) and, as a consequence, also the $\bdelta$ matrix and predictions $\by$ are now splitted in unary and binary matrices ($\bdelta_U$ and $\bdelta_B$ for the residues, $\by_U$ and $\by_B$ for the final predictions). 

% Indeed, the i$^th$ KE takes into account the predictions made by the 



% \subsubsection{\TODO{Architecture of Relational KE}}
% \TODO{
% \kenn\ considers unary and binary clauses separately, by adopting two separate instantiations of the KE architecture, namely
% KE$_u$ and KE$_b$. The former computes the contributions of the clauses in $\clauses_u$ and the latter computes the contributions of the clauses in $\clauses_b$.
% The structure of KE$_u$ and KE$_b$ is the same (shown in Fig.~\ref{fig:KE}). The only difference between the two is that KE$_u$ takes in input the pre-activations on unary predicates in $\bz_U$, while KE$_b$ takes in input the pre-activations of both unary and binary predicates. Indeed, binary clauses can contain both unary and binary predicates.

% Fig.~\ref{fig:relational_kenn}(b) shows the architecture of the Realtional KE. As mentioned before, the unary knowledge $\clauses_U$ is applied directly to $\bz_U$ using the KE$_U$ module. 
% % \TODO{spostare prima pre-elab spiegando zm (e dopo dire che la uso per binary knowledge)}
% The binary knowldge is enforced on a bigger matrix $\bz_M$, which contains all the binary predicates as well as the unary predicates applied on both $x$ and $y$. Such a matrix is calculated by a pre-elaboration step which copies the multiple times the grounded atoms of $\bz_U$ inside the right position of $\bz_M$. As an example, the pre-activation of $Smoke(a)$ (red in Fig.~\ref{fig:relational_kenn}(b)), is copied in three different positions inside $\bz_M$.

% KE$_B$ is applied on $\bz_M$ using the binary knowldge $\clauses_B$. The returned $\delta_M$ matrix contains multiple residues for the same atom, since each grounded atom could be included in multiple groundings of the same clauses (hence, different rows of the matrix). For instance, in Fig.~\ref{fig:relational_kenn}(b), blue values represent the changes to be applied to $Smoke(a)$. A post-elaboration step is used to sum up such values together with the changes proposed by KE$_U$ and store them inside $\bdelta_U$.
% }








The RKE has the same role as the KE in the unary case. However, it is capable to consider also binary predicates. When binary knowledge is available, additional steps are required since the independence between object can not be assumed anymore.

Let $\clauses_U$ be the set of unary clauses and $\clauses_B$ the set of binary clauses. The prior knowledge is now defined as $\clauses = \clauses_U \cup \clauses_B$.
% The idea is to apply the KE to these two sets separately: Equation~\ref{eq:final_intepretation_unary} can be decomposed using the new defined partition of the knowledge:
% \begin{equation}
% 	y_A = \sigma \left( z_A + \sum_{c \in \clauses_U[\C]} w_c \cdot \delta_{c,A} + \sum_{c \in \clauses_B[\C]} w_c \cdot \delta_{c,A} \right)
%     % &= \sigma(\bz + \bdelta_U + \bdelta_B)
% 	\label{eq:final_intepretation_binary}
% \end{equation}
% where $A$ is a grounded atom (here we use $A$ instead of $P(a)$ since this is true for no a grounded unary or binary predicate).
% % where $\bdelta_U$ and $\bdelta_B$ are the changes to be applied on unary and binary predicates respectively.
The idea is to apply the KE to these two sets separately. Equation~\ref{eq:final_intepretation_unary} can be decomposed using the new defined partition of the knowledge:
$
	y_A = \sigma \left( z_A + \sum_{c \in \clauses_U[\C]} w_c \cdot \delta_{c,A} + \sum_{c \in \clauses_B[\C]} w_c \cdot \delta_{c,A} \right)
    % &= \sigma(\bz + \bdelta_U + \bdelta_B)
	% \label{eq:final_intepretation_binary}
$, 
where $A$ is a grounded atom (i.e. $P(a)$ or $P(a,b)$, depending on the arity of $P$).
% where $\bdelta_U$ and $\bdelta_B$ are the changes to be applied on unary and binary predicates respectively.
We define $\bdelta_{\clauses_U}$ as the changes deriving from unary clauses:
\begin{equation}
    \delta_{\clauses_U,P(a)} = \sum_{\substack{c \in \clauses_U\\ P(x) \in c}} w_c \cdot \delta_{c[a],P(a)}
	\label{eq:ku_pa}
\end{equation}
Similarly, $\bdelta_{\clauses_B}$ are the changes calculated from $\clauses_B$.

Notice that the approach defined so far can be directly applied to the unary knowledge $\clauses_U$ to calculate $\bdelta_U$ since traditional KE can manage unary knowledge. Indeed, internally the RKE contains a standard KE which manages the unary clauses. 

We need to define a strategy to deal with binary clauses. Indeed, when a clause $c$ contain two variables, 
% the same ground atom may occour in multiple groundings of the clause.
a grounding of a unary predicate may occur in multiple groundings of $c$.
For instance, consider the clause of Eq.~\ref{eq:clause}.
The two groundings $c_{SF}[a,b]$ and $c_{SF}[b,c]$ share a common grounded atom: $Smoker(b)$. 
% For this reason, it is not possible to use a single matrix to store all the atoms without repetitions.
For this reason, when dealing with the predictions of a unary predicate in a relational domain, we need to account for such repetitions:
\begin{equation}
    \delta_{\clauses_B,P(a)} = \sum_{b \neq a} \Big( \sum_{\substack{c \in \clauses_B\\ P(x) \in c}} w_c \cdot \delta_{c[a,b],P(a)} +  \sum_{\substack{c \in \clauses_B\\ P(y) \in c}} w_c \cdot \delta_{c[b,a],P(a)} \Big)
	\label{eq:kb_pa}
\end{equation}

Putting all together, the predictions $y_{P(a)}$ for a grounded unary predicate $P$ are defined as:
\begin{equation}
	y_{P(a)} = \sigma(z_{P(a)} + \delta_{\clauses_U,P(a)} + \delta_{\clauses_B,P(a)} )
    % &= \sigma(\bz + \bdelta_U + \bdelta_B)
	% \label{eq:final_intepretation_binary}
	\label{eq:y_pa}
\end{equation}

The predictions for a binary predicate $R$ are easier to be computed since they can be found only in binary clauses and any possible grounding of $R$ can be found in only one corresponding grounding of each clause
$y_{R(a,b)} = \sigma(z_{R(a,b)} + \delta_{\clauses_B,R(a,b)})$, 
with
\begin{equation}
	\delta_{\clauses_B,R(a,b)} = \sum_{\substack{c \in \clauses_B\\ R(x,y) \in c}} w_c \cdot \delta_{c[a,b],R(a,b)}
	\label{eq:kb_rab}	
\end{equation}

% A figure summarizing the entire architecture of \kenn\ on relational data, together with some implementation details about the RKE, can be found in Appendix~\ref{ap:rel_kenn}. % 
 
\subsection{\new{Time complexity}}
\new{Here we analyze the time complexity of an RKE layer with respect to domain size $m$, number of predicates $|\P|$, and number of rules $|\clauses|$. We also assume the maximum number $L$ of literals in a clause to be a small constant.
	
Let us first analyze the time complexity for calculating the $\delta_{c[a]}$ used in Equations~\ref{eq:ku_pa}, and \ref{eq:kb_pa}. Each $\delta_{c[a],P(a)}$ can be calculated in time $O(1)$ (see Equation~\ref{eq:deltac}). 
% Assuming the maximum number $L$ of literals in a clause to be a small constant, 
Computing $\delta_{c[a]}$ also requires constant time. The sum of Equation~\ref{eq:ku_pa} require time $O(|\clauses|)$, which is the time necessary to compute $\delta_{\clauses_U,P(a)}$. Note that neural networks are usually run on GPUs, where the computations can be parallelized. Assuming enough parallel processes ($|\clauses|$ in this case), a sum can be performed in a time logarithmic with respect to the number of addends, and complexity for $\delta_{\clauses_U,P(a)}$ becomes $O(log(|\clauses|))$. Finally, Equation~\ref{eq:ku_pa} needs to be calculated for all the grounded unary predicates $P(a)$, for a total time of $O(m \cdot |\P| \cdot |\clauses|)$ in a single process, and $O(log(|\clauses|))$ with multiple parallel processes (each of the grounded atom can be considered independently from the others). With a similar reasoning, we found the time complexity of Equations~\ref{eq:kb_pa} and \ref{eq:kb_rab} to be $O(m^2 \cdot |\P| \cdot |\clauses|)$. Note that with enough parallel processes we can compute all the deltas in $O(log(m) + log(|\clauses|))$.

% Note that each $\delta_{c[a]}$ and $\delta_{c[a,b]}$ can be calculated in parallel since the previous formalization assumes independence between each grounded clause. As a consequence, if there are enough parallel processes, the time consumed for grounding the clauses and finding the corresponding residues is constant. On the other hand, the summation in equations 6 can be performed in time logarithmic in the number of addends, i.e., in $O(log(|\clauses_U|))$. Similarly, the summations of equation \todo{7} can be performed in $O(log(|\clauses_B| * n)) = O(log(|\clauses_B|) + log(\todo{n}))$, where n is the number of domain elements. Finally, the summation in equation 9 can be calculated in time $O(log(|\clauses_B|))$. In summary, when running on a GPU, and assuming enough kernels available, we can expect the computations of the RKE layer to be performed in time $O(log(|\clauses_U|) + log(|\clauses_B|) + log(n))$.
}


\subsection{Treatment of dependencies among the rules}
\label{sec:reasoning}
\new{In the previous section we showed the efficacy of the method in terms of execution time, which can be achieved thanks to the assumption of independence. However, when this assumption is violated, \kenn\ does not provide any guarantees on the satisfaction of the knowledge.}
% , increasing the truth value of a subset of the clauses.
\new{As an example,} suppose that we have two grounded clauses $c_1: \lnot A \lor B$ and $c_2: \lnot B \lor C$ with their respective clause enhancers CE$_1$ and CE$_2$, where $A$, $B$ and $C$ are grounded unary or binary predicates. The atom $B$ appears in both clauses with opposite signs.
Since the CE increase the highest literal value (see Eq.~\ref{eq:phi}), if $A < B$~\footnote{With an abuse of notation, we use the atoms symbols to refer also to their truth value} and $C < \lnot B$, then CE$_1$ increases $B$ and CE$_2$ decreases it. As a consequence, the satisfaction of only one between $c_1$ and $c_2$ is increased. Furthermore, the satisfaction of the entailed clause $\lnot A \lor C$ is also not improved. 

% In this scenario, the two CEs could both increase and decrease the value of predicate $B$ and leave unalterated $A$ and $C$. As a consequence, one between $c_1$ and $c_2$ would not be satisfied, as well as the clause $\lnot A \lor C$, which is a consequence of the two. 

%  arises when $A < B$ and $C < \lnot B$, since a CE increases the highest literal value (see Eq.~\ref{eq:phi}).
% can be alleviated by stacking multiple KEs on top of each other. 
For any grounded atom $G$, lets define $G^{(0)}$ as its initial prediction and $G^{(i)}$ as the prediction of the $i^{th}$ KE layer. Moreover, suppose that all KEs share the same clause weights $w_1$ and $w_2$ (for $c_1$ and $c_2$ respectively). From Equations~\ref{eq:final_intepretation_unary} and \ref{eq:deltac} we can derive $B^{(1)} = B^{(0)} + w_1 - w_2$, and $\lnot B^{(1)} = \lnot B^{(0)} + w_2 - w_1$. If $w_1 \geq w_2$, then 
$A^{(1)} = A^{(0)} < B^{(0)} \leq B^{(1)}$.
As a consequence, the first rule will increase again $B$ even at the next KE layer. On the other hand, the value of $\lnot B$ is reduced, which means that there is an increased chance for $C^{(1)} > \lnot B^{(1)}$, which would solve the problem since CE$_2$ would increase $C$ instead of $\lnot B$. Notice that, since the weights are the same at each level, it is always true that $\lnot B^{(i+1)} \leq \lnot B^{(i)}$, meaning that with enough KE layers both clauses' satisfaction will be increased (and as a consequence, also their entailments).
%  Notice also that the same type of reasoning can be applied when $w_1 \leq w_2$.


\new{The problem analyzed in this section } becomes even more relevant in relational domains since in these contexts an atom can be shared not only by multiple clauses but also by different groundings of the same clause (for instance, in $c_{SF}[a,b]$ and $c_{SF}[b,c]$). For this reason, in these contexts stacking multiple RKEs is recommended (more details in Section~\ref{sec:results}).

% \todo{Another perspective on this solution comes from the graph representation. From this point of view, an RKE changes the predictions of one node of the graph based exclusively on the values of its neighbors and by stacking multiple RKEs we allow for the propagation of the constraints like in Graph Convolutional Networks~\cite{GCN}.(Eliminare paragrafo?)}







% \new{ From the graph representation point of view, this limitation arises from the fact that an RKE changes the predictions of one node of the graph based exclusively on the values of its neighbors.}
% For this reason, in these contexts stacking multiple RKEs is recommended.
% Another perspective on this solution comes for the graph representation. 
% \new{From this point of view, we need a method to propagate the constraints to \todo{farther} nodes.}
% a RKE changes the predictions of one node of the graph based exclusively on the values of its neighbors. 
% From this perspective, \new{a feasible solution consist of stacking multiple RKEs on top of each other. Similar to what happens in Graph Convolutional Networks~\cite{GCN}, this strategy allows for the propagation of the constraints inside the graph. In the example provided above, ...}

% Moreover,
% that here we explicitly represent the architecture with multiple RKEs stacked on top of each other. Indeed, 
% the problem highlighted in Section~\ref{sec:reasoning} becomes even more relevant in relational domains since in these contexts an atom can be shared not only by multiple clauses, but also by different groundings of the same clause (for instance, in $c_{SF}[a,b]$ and $c_{SF}[b,c]$). 
% For this reason, in these contexts stacking multiple RKEs is recommended.
% Another perspective on this solution comes for the graph representation. From this point of view, a RKE changes the predictions of one node of the graph based exclusively on the values of its neighbors. For this reason, by stacking multiple RKEs we are allowing for the propagation of the constraints in a similar manner as Graph Convolutional Networks~\cite{GCN}.





% \subsubsection{Implementation \todo{move inside evaluation ...}}


% \kenn\ has been implemented as a library for Python 3. It is based on TensorFlow 2 and Keras and it 
% is available as an open-source project on Github\footnote{\href{https://github.com/DanieleAlessandro/KENN2}{https://github.com/DanieleAlessandro/KENN2} \todo{anonimizzare codice e mandarlo come supplementary material}}.


% using a \TODO{matrix ...in parallel} is problematic since the values returned by the CE would not be aggregated, and we would end up with multiple changes proposed for the same atom.

% Figure\TODO{...} shows such a matrix for the Smoking Friends example:

% \TODO{immagine}







% The idea now is to apply KE to the two sets $\clauses_U$ and $\clauses_B$ separately.
% % % : the changes to be applied on binary predicates comes only from binary clauses, while the changes on unary clauses depends on both unary and binary clauses.
% In the first case, KE can be called directly on $\U$ using only the unary knowledge $\clauses_U$ since here all the clauses involves a single variable and only unary predicates (all inside $\U$).
% % This can be done since $\U$ contains only unary predicates and it represents the data in the same way \TODO{of $\bz$ for the multi-label version of \kenn.} 
% The output of KE is a matrix that collects the changes to be applied to $\U$ based on unary clauses $\clauses_U$. We call it $\delta \U^u$ to distinguish it from $\delta \U^b$ (the changes to apply to matrix $\U$ based on binary clauses).

% At this point we also need to increase the satisfaction of binary clauses. To do this, the idea is to reduce the binary case to the unary one so we can still use the KE as defined in Section\TODO{....}. Next sections dive more deeply into this approach.





% As previously mentioned, previous to this work \kenn\ could only be used in the presence of unary predicates. This is bacause it makes use of a 

==> Relational KENN/state_of_the_art.tex <==
\section{Related works}
\label{ch:rel_works}

Many previous works attempt to combine learning models with logical knowledge. Among them there is 
% particularly relevant are works on 
Statistical Relational Learning (SRL), a subfield of Machine Learning that aims at applying statistical methods in domains that exhibit both uncertainty and relational structure \cite{introduction_SRL}. \new{Generally speaking, SRL deals with the knowledge either by combining logic rules with probabilistic graphical models (e.g., Markov Logic Networks~\cite{MLN}, and \emph{Probabilistic Soft Logic} (PSL)~\cite{PSL}) or by extending logic programming languages to handle uncertainty (e.g., ProbLog \cite{problog}).}

% In this category, there is Markov Logic Networks~\cite{MLN}, which uses weighted FOL rules as a template for building Markov Random Fields \cite{MRF}.
% A similar framework is \emph{Probabilistic Soft Logic} (PSL)~\cite{PSL} which uses a continuous relaxation of the variables to gain efficiency. 

% Neither MLN, nor PSL can deal with real values features. To obviate at this limitation, an extension of MLN, called Hybrid Markov Logic Networks (HMLN), has been introduced in \cite{HMLN}. HMLN differs from MLN for its ability to represent continuous variables.

% Generally speaking, SRL deals with the knowledge either by combining logic rules with probabilistic graphical models (as in the previously mentioned work) or by extending logic programming languages to handle uncertainty, like in the case of ProbLog \cite{problog}.


The recent achievements of deep learning methods lead to a renewed interest in another line of research, called Neural-Symbolic Integration, which focuses on combining neural network architectures with logical knowledge~\cite{neural_symbolic}.
% Neural networks are perfectly suited for pattern recognition, even in the presence of noisy data. They are particularly good at mapping low-level perceptions to more abstract concepts (for instance, going from images to classes). However, it is hard for a NN to reason with this high-level abstractions. Furthermore, NNs are demanding in terms of training data. On the other hand, pure logical approaches are not efficient at learning from low-level features and they struggle in the presence of noise. Nevertheless, they perform well on reasoning with highly abstract concepts and on learning from a small number of samples. Given these opposite strengths and weaknesses, it is not a surprise that a lot of interest has been drawn towards Neural-Symbolic systems. Indeed, the goal is to combine these two paradigms to obtain the best of the two worlds.
This can be achieved in multiple ways depending on the role of the knowledge. For instance, works like 
TensorLog~\cite{tensorlog}, Neural Theorem Prover (NTP)~\cite{NTP1,NTP2}, DeepProbLog~\cite{deepproblog}, Neural Logic Machines~\cite{NLM}, and NeuralLog~\cite{NeuralLog}
focus on the development of differentiable approaches for reasoning, which can be used in combination with neural networks. Another line of research comes from methods like 
$\partial$ILP~\cite{dilp}, \cite{rule_induction}, and Neural Logic Rule Layer (NLRL)~\cite{NLRL}. In these cases, the goal is to learn general knowledge from the data, either from scratch or by refining an initial knowledge. Finally, more related to our purposes, some methods focus on learning in the presence of prior knowledge, which acts as additional supervision. In this section, we are going to focus on these types of methods, since \kenn\ falls in this category.

% On the contrary, in our case, we are interested in methods that use the logic in an opposite direction: the knowledge here is given a priori, and the goal is to use such knowledge as a sort of additional supervision to guide the learning.

There are mainly two approaches for learning in the presence of prior knowledge: the first consists of treating logical rules as constraints on the predictions of the neural network. The problem is reduced to maximize the satisfiability of the constraints and can be efficiently tackled by adding a regularization term in the Loss function which penalizes the unsatisfaction of the constraints. The second approach is to modify the neural network by injecting the knowledge into its structure.

% One approach for learning in presence of Prior Knowledge is to treat logical rules as constraints on the predictions of the Neural Network. The problem is reduced to maximize the satisfiability of the constraints and can be efficiently tackled by adding a regularization term in the Loss function which penalizes the unsatisfaction of the constraints.

% \subsubsection{Regularization approaches}

Two notable examples of regularization approaches are \emph{Logic Tensor Network} (LTN)~\cite{LTN} and \emph{Semantic Based Regularization} (SBR)~\cite{SBR}. Both methods maximize the satisfaction of the constraints, expressed as FOL formulas, under a fuzzy logic semantic. 
% As mentioned above, LTN can be also classified as a DR approach. 
% Although it was shown to be able to perform reasoning, 
% \TODO{The greater achievements of this model} have been obtained in the KGL paradigm, in particular in the context of image interpretation \cite{IvanThesis,DonadelloSG17}. 
A similar strategy is employed also by \emph{Semantic Loss Function}~\cite{semantic_loss}, but instead of relying on fuzzy logic, it optimizes the probability of the rules being true. Nevertheless, this approach is restricted to propositional logic. \cite{dl2} introduces DL2.
%  which is also a method that includes logical knowledge through the Loss function. 
Nonetheless, it can be used only in the context of regression tasks, where the predicates correspond to comparison constraints (e.g. $=$, $\neq$, $\leq$).
%  between terms that can be either output of the network or constants.
MultiplexNet~\cite{MultiplexNet} also uses comparison constraints, but it is not restricted to them. In this case, the interest is in safety-critical domains where complete satisfaction of the constraints is desirable and the knowledge is expressed in disjunctive normal form (DNF).
% Each term of the DNF is used to propose a possible transformation of the NN's outputs and a latent variable is used to select the best one. The chosen transformation is used to create a regularization term in the Loss. 
\cite{adversarially} also proposes a method that regularizes the Loss, but they focus on a specific task of Natural Language Processing. Their approach differs from the others because it makes use of adversarial examples to calculate the regularization term.
% : first, it generates samples that minimize the satisfaction of the constraints, then it optimizes the NN to increase their satisfaction. 
Finally, in \cite{semi_supervised} 
% it is again proposed a regularization technique. This time, 
% a regularization technique is used for a Semi-Supervised Learning task, and 
the regularization term is calculated from the unlabelled data.

In~\cite{harnessing}, a distillation mechanism is used to inject FOL rules.
% : a student network is trained both on predicting the correct labels and emulating a teacher network; the teacher network is obtained by reducing the KL-Divergence with the student network and at the same time optimizing the satisfaction of the rules. 
While this approach seems different from the previous ones, we argue that it can be also considered as a method based on regularization, since a teacher network (which encodes the rules) is used to regularize the Loss applied to a student network.
Finally, in~\cite{old_dog}, a new technique is defined which adds the knowledge at the level of the labels by modifying them after each training step. 
% The approach is quite general, but it does not provide any guarantees on the convergence. 

% Again, even if this method is different from the previous ones, the effect on learning should be similar: in the previous cases, the Loss is combined with a regularization term to find a balance between fitting the correct labels and satisfying the knowledge; here, 
% this is done indirectly by modifying the labels to increase the satisfaction of the knowledge.


% \subsubsection{Model based approaches}
Model-based approaches work pretty differently from the methods seen so far. The main difference lies in the way logic formulas are used:
%  in model-based approaches 
the knowledge becomes part of the classifier.
%  instead of being enforced during training.
Instead, approaches based on regularization force the constraints satisfaction solely at training time. As a consequence, there are no guarantees that they will be satisfied at inference time as well. A way to reduce such a problem is to enforce the constraints not only during training but also at inference time~\cite{SBR_collective}. However, notice that in this case the time complexity of inference is increased since the back-propagation needs to be used even in this case. On the other hand, methods that inject knowledge directly into the model structure are naturally capable of enforcing the knowledge at inference time.
% \TODO{, since the rules are directly codified by the NN}.

% \TODO{



% \kenn\ englobes the knowledge into the network in a very different way than SBR
% %  and LTN
% . As already discussed, SBR 
% % and LTN 
% acts on the Hypothesis Space (HS) by changing the associated loss function according to the constraint.

% The approach of 
% % LTN and
% SBR is equivalent to ``remove'' solutions from the HS that do not satisfy the constraints by penalizing them during training (they are not really removed, but difficult or impossible to reach because of the penalty given by the Loss function), while in \kenn\ the approach is the opposite: new solutions are added to the Hypothesis Space (HS) by a new additional layer, called \emph{Knowledge Enhancer}. 

% }

Another possible advantage of model based methods is the possibility to learn a weight that codifies the importance of a logical rule directly from the data. This is no possible at all with methods based on regularization, since the logical formulas are directly codified inside the Loss function. As a consequence, if some rule weight is available, it must be added as a hyper-parameter.

Among the few methods that admit learnable weights associated with the logic formulas there is \kenn. This makes it suitable for scenarios where the given knowledge contains errors or when rules are softly satisfied in the real world but it is not known in advance the extent to which they are correct.
\kenn\ injects knowledge on top of the NN model through an additional layer which increases the satisfaction of the constraints in a fuzzy logic semantic. 


Another approach
% that directly encodes the knowledge into the structure of the model 
is provided by Li and Srikumar who recently proposed a method that codifies the logical constraints directly into the neural network model~\cite{augmenting}. However, they restrict the rules to implications with exactly one consequent and they do not provide the possibility to learn clause weights, which in their system are added as hyper-parameters. 

Going in the same direction, \cite{RNM} proposed Relational Neural Networks (RNM). RNM can be also inserted in the set of approaches that add the logic directly into the model and, as the best of our knowledge, it is the only method other than \kenn\ which is capable of integrating logical knowledge with a neural network while learning the clause weights. RNM integrates a neural network model with a FOL reasoner. This is done in two stages: in the first one, the NN is used to calculate initial predictions for the atomic formulas; in the second stage a graphical model is used to represent a probability distribution over the set of atomic formulas. To obtain the final predictions a Maximum a Posteriori (MAP) estimation is performed, finding the most probable assignment to the grounded atoms given the output of the NN and the set of constraints. At a high-level RNM approach is similar to \kenn, since in both cases a NN makes initial predictions and a post elaboration step is applied to such predictions to provide the final classification. However, RNM requires to solve an optimization problem at inference time and after each training step. This has the advantage of considering all the logical rules together at the same time at the expense of an increased computational effort. Contrary, in \kenn\ each rule is considered separately from the others, and the second stage is directly integrated inside the model as a differentiable function that can be trained end-to-end with the NN. However, 
% one could argue that
with this strategy there could be some contradictory changes when combining multiple clauses with the same predicates. We will further analyze this aspect in \new{Section~\ref{sec:reasoning}, proposing a strategy to handle this limitation. Moreover, in Section~\ref{sec:collective}, we analyze this strategy empirically.}








==> architecture.tex <==
\section{\kenn\ architecture}
\label{sec:architecture}
% This chapter is divided into two main sections: in the first one, it is defined a simple architecture for \kenn\ for multi-label classification tasks; in the second one we will introduce how to extend it for relational data.

% \section{Architecture}
% \label{sec:architecture}
As explained in Section~\ref{sec:kenn}, the core component of \kenn\
is in the \boost . In \kenn\ the \boost\ for a certain clause $c$ is
implemented by an architecture called \emph{Clause Enhancer} (CE), which is a
module instantiated that computes $\delta_c$ according to Equation~\eqref{eq:deltac}. 
Figure~\ref{fig:CE} shows the details of the architecture of the CE. 

% \subsection{Clause Enhancer}

\begin{figure}[H]
  \centering
	\input{tikz/CE}
	\caption{Clause Enhancer for $A \lor \lnot B$, where $A$ and $B$ are grounded atoms}
	\label{fig:CE}
\end{figure}

The CE receives as input a vector containing the preactivations generated by the base NN and it selects the right literals, returning $\bz_c$, the preactivations of the literals of clause $c$.
% the literals occurring in $c$ obtaining $\bz_c$, the preactivations of the literals of clause $c$. 
Then, Equation \ref{eq:delta_wc_s} of $\delta_s^w$ is applied. 
% Intuitively, the idea is that, in order to satisfy a clause, at least one of its literal must be true. The softmax function act as a selector for the most promising true literal, that is the one with highest supporting evidences (biggest preactivation).} 
The term $w_c$ is a positive weight associated to clause $c$ that represents the strength of $c$: the higher the $w_c$, the bigger the contribution of the clause in the final predictions. As opposed to methods based on the regularization of the Loss, $w_c$ is not a hyper parameter. On the contrary, it is a parameter of the model that is learned during training. This means that \kenn\ can discover the importance of each clause based on the data. As a special case of this behavior, it is possible for \kenn\ to learn to ignore clauses by setting $w_c$ to zero, making clause $c$ irrelevant for the final predictions.

The final step of the CE is a post elaboration that projects the proposed changes on the literals into changes to be applied on the atoms according to equation \ref{eq:deltac}.
% This operation corresponds to the Equation~\ref{eq:phip}.
%  for calculating $\delta_c$.

% \subsection{Knowledge Enhancer}

The outputs of the CEs are combined inside the \emph{Knowledge Enhancer} (KE), which is the final layer of \kenn\ model. Figure~\ref{fig:KE} shows the architecture of KE, which calculates the final interpretation as in Equation~\ref{eq:final_intepretation}.
%  Notice that a CE is instantiated for each grounded clause $c \in \G(\clauses, \C)$.

\begin{figure}[H]
	\centering
	\input{tikz/KE}
	\caption{Knowledge Enhancer architecture. It implements Equation~\ref{eq:final_intepretation} by summing the deltas values of each clause enhancer (one per grounded clause) with the initial preactivations $\bz$ and applying the logistic function }
	\label{fig:KE}
\end{figure}


% \subsection{Working with batches of data}
% In the architecture defined so far, since all the grounded atoms are inside the vector $\bz$, there are multiple instantiation of the same CE for each clause $c \in \clauses$, one for each grounding of $c$. For instance, in Figure~\ref{fig:KE_matrix}(a), the CE for clause $c: \lnot S(x) \lor C(x)$ is instantiated two times, one for object $a$, another for object $b$. 

% In many scenarios we want to use batches of data, which would require to modify the structure of the model graph for each batch, in particular after each training step, since the groundings are constantly changing and for each grounding a different CE is instantiated. Notice that, even if the CEs are different, the internal operations are the same and the only change is the provided input. For these reasons, we want to instantiate a single CE for each clause $c$ which works in a single batch containing all possible groundings of $c$.

% If the groundings involve a single object, a simple solution is to define $\bz$ as a matrix instead as a vector, where columns represent predicates and rows individuals. More in details, $\bz$ is now defined as a matrix such that the element $z_{ij}$ contains the preactivation of $P_j(o_i)$, with $P_j$ the $j^{th}$ predicate and $o_i$ the $i^{th}$ object. 
% Notice that this kind of representation is common when working with neural networks since the columns (predicates) correspond to the labels and the rows (groundings) to the samples. 

% Figure~\ref{fig:KE_matrix}(b) shows the overall idea. The CE is defined as before, but now it takes as input a matrix and it acts on each row separately. This can be done only if the same atom does not appear in multiple rows, since the changes are applied independently to each row and are not aggregated together. This property always holds with clauses that
% % have only unary predicates and 
% involve a single variable.
% % : we call this type of clauses \emph{unary}. In contrast, a clause that contains two variables is referred as a \emph{binary} clause. We define $\clauses_U$ as the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge can be described as $\clauses = \clauses_U \cup \clauses_B$.
% % For simplicity, in this thesis we don't take into account clauses with higher ariety. However, the proposed approach can be used with predicates and clauses with any number of variables.

% % As mentioned above, when dealing with unary clauses the approach of Fig~\ref{fig:KE_matrix}(b) can be used. 

% When a clause contain multiple variables, the same ground atom may occour in multiple groundings of the clause. 
% For instance, consider the clause 
% $$c: \lnot Smoke(x) \lor \lnot Friends(x,y) \lor Smoke(y)$$
% The two groundings $c[x/Alice,y/Bob]$ and $c[x/Bob,y/Carl]$ share a common grounded atom: $Smoke(Bob)$. For this reason, using a unique CE for $c$ is problematic since the values returned by the same CE are not aggregated, and we would end up with multiple changes proposed for the same atom.

% In the next sections, we will present the architecture of \kenn\ that can be used to instantiate a single CE even in relational domains, i.e. when dealing with predicates with arity greater than one.



% \begin{figure}[H]
% 	\centering
% 	\input{tikz/KE_matrix}
% 	\caption{KE applied on a Prior Knowledge consisting of a single clause $c$: $\lnot S(x) \lor C(x)$ applied on a domain of two objects ($a$ and $b$): (a) using a vector with all the grounded atoms, each grounding of $c$ is managed by a different CE.  Notice that the changes proposed by the first CE are zero for $C(b)$ and $S(b)$ while the second CE returns the value zero for the other two atoms: the two grounded clauses are independent; (b) using a matrix with a row for each grounding: all the grounding of $c$ are managed by the same CE, which operates in parallel on each row of the matrix. This is more convenient when dealing with mini-batches and results in a more efficient implementation.}
% 	\label{fig:KE_matrix}
% \end{figure}


% \subsection{KE for relational data}
% %\subsubsection{Unary and binary clauses}
% %\label{sec:SRL_representation}

% Maintaining a single vector with all the grounded atoms as in Section~\ref{sec:architecture} could lead to an inefficient implementation since it forces to create multiple CEs for each clause. This means that it requires to reset the computational graph every time new data is provided. On the other hand, in the approach of Fig.~\ref{fig:KE_matrix}(b), for each clause only a CE is instantiated and it can work in parallel on all the groundings of the clause. This has two advantages: it simplifies the usage of batches during training, and CEs' internal calculations are implemented as matrix operations, which are particularly efficient when working with a GPU. 

% However, such an approach can be applied with clauses that involve a single variable: we call this type of clauses \emph{unary}. In contrast, a clause that contains two variables is referred as a \emph{binary} clause. For simplicity, we don't take into account clauses with higher arity. Notice however that the proposed approach can be used with predicates and clauses with any number of variables.

% % We define $\clauses_U$ as the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge can be described as $\clauses = \clauses_U \cup \clauses_B$.
% % For simplicity, in this thesis we don't take into account clauses with higher ariety. However, the proposed approach can be used with predicates and clauses with any number of variables.

% % As mentioned above, when dealing with unary clauses the approach of Fig~\ref{fig:KE_matrix}(b) can be used. 


% % We introduce a classification for clauses based on the number of variables they contains: a clause is unary if it contains only one free variable, binary if it contains two variables. 

% Let $\clauses_U$ be the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge is now defined as $\clauses = \clauses_U \cup \clauses_B$.

% The idea now is to apply the KE to these two sets separately: Equation~\ref{eq:final_intepretation} can be decomposed using the new defined partition of the knowledge:
% \begin{equation}
% 	\begin{split}
% 	\by'&= \sigma \left(\bz + \sum_{c \in \G(\clauses_U)} \bdelta_c + \sum_{c \in \G(\clauses_B)} \bdelta_c \right)	
% 	\end{split}
% 	\label{eq:final_intepretation_binary}
% \end{equation}

% Notice that the approach defined in the previous section with a single CE for each clause can be directly applied to the unary knowledge $\clauses_U$. We need to define a strategy to deal with binary clauses. 

% % The idea now is to apply KE to the two sets $\clauses_U$ and $\clauses_B$ separately.
% % % % : the changes to be applied on binary predicates comes only from binary clauses, while the changes on unary clauses depends on both unary and binary clauses.
% % In the first case, KE can be called directly on $\U$ using only the unary knowledge $\clauses_U$ since here all the clauses involves a single variable and only unary predicates (all inside $\U$).
% % % This can be done since $\U$ contains only unary predicates and it represents the data in the same way \TODO{of $\bz$ for the multi-label version of \kenn.} 
% % The output of KE is a matrix that collects the changes to be applied to $\U$ based on unary clauses $\clauses_U$. We call it $\delta \U^u$ to distinguish it from $\delta \U^b$ (the changes to apply to matrix $\U$ based on binary clauses).

% % At this point we also need to increase the satisfaction of binary clauses. To do this, the idea is to reduce the binary case to the unary one so we can still use the KE as defined in Section\TODO{....}. Next sections dive more deeply into this approach.

% \subsubsection{Representing relational data in tables}
% \label{sec:relational_representation}

% To represent relational data, \kenn\ adopts two matrices, denoted by $\U$ and $\B$, which could be seen as tables of a relational database. Fig.~\ref{fig:representation} shows this representation using the classical Smoker-Friends-Cancer example: there is a domain composed of three objects (persons) $O = \{o_0, o_1, o_2\}$, two unary predicates ($S$ and $C$, which stand for $Smoking$ and $Cancer$) and one binary predicate $F$ ($Friends$)). Fig.~\ref{fig:representation}(a) shows the graph representation with nodes and edges labelled with the unary and binary predicates respectively. In this particular example the graph has no self-loops, meaning that $Friends(x,x)$ is not taken into account. Please notice that this limitation is specific for this example since everyone is assumed to be friends of himself a priori. However, in general, \kenn\ can work with self-loops.

% Fig.~\ref{fig:representation}(b) shows the data structure used to encode the graph of Fig.~\ref{fig:representation}(a): matrix $\U$ contains as many rows as objects in the domain and as many columns as unary predicates plus a key column $i$, which could be interpreted as a primary key for the table $\U$. Intuitively, 
% the $j^{th}$ row of $\U$ contains the preactivations of the unary predicates applied on the $j^{th}$ object,
% i.e., $\U_j=(z_{P_1(o_j)},\dots,z_{P_n(o_j)})$. 

% Matrix $\B$ contains one row for every pair of objects to which we want to apply
% a binary predicate. 
% Notice that we might not want to include all the pairs of objects in $\B$, because the application of binary predicates of some pairs might be meaningless. For instance, as already mentioned, the $Friends$ predicate applied to $(a,a)$ is not interesting.
% $\B$ has one column for each binary predicate and other two columns $s^x$ and $s^y$ that indicate the first and the second component of the
% pair. In the relational database analogy they can be seen as foreign keys to table $\U$. As with $\U$, each row represents a different grounding of the predicates, with the difference that in this case the predicates are binary and the variables to be substituted are two. More precisely, $\B_{i,j}$ corresponds to the value of predicate $B_j$ for the substitution $(x / o_{s^x_i}, y / o_{s^y_i})$:
% $$\B_{i,j} = B_j(o_{s^x_i},o_{s^y_i})$$

% For instance, in Fig.~\ref{fig:representation}(b): $s^x_0 = 0$ and $s^y_0 = 1$, which means that row $0$ of matrix $\B$ is referring to the pair of objects $(o_0,o_1)$.


% \begin{figure}
% 	\centering
% 	\input{tikz/rel_representation}
%     \caption{
% 		Relational data representation: in this example, three objects ($o_0$, $o_1$ and $o_2$), two unary predicates ($S$ and $C$) and only one binary predicate ($F$). (a): the graph representation; (b): the representation used by \kenn: matrixes $\U$ and $\B$ can be interpreted as tables of a relational database: $\U$ contains all the groundings of unary predicates and an index column $i$ which correspond to the `primary key' of the table; matrix $\B$ contains the groundings of binary predicates together with columns $s^x$ and $s^y$ which corresponds to ``foreign keys''  to table $\U$.
% 		Values refer to preactivations of atoms' truth values.}
%     \label{fig:representation}
% \end{figure}

% \def\alice{a}
% \def\bob{b}
% \def\chris{c}

% \kenn\ considers unary and binary clauses separately, by adopting two separate instantiations of the KE architecture, namely
% KE$_u$ and KE$_b$. The former computes the contributionsof the clauses in $\clauses_u$ and the latter computes the contributions of the clauses in $\clauses_b$.
% The structure of KE$_u$ and KE$_b$ 
% is the same (shown in the right of Figure~\ref{fig:KE_matrix}). The only difference between the two is that KE$_u$
% takes in input the preactivations on unary predicates in $\U$,
% while KE$_b$ takes in input the preactivations of both unary and binary predicates. Indeed, binary clauses can contain unary predicates and
% we need a method to encode unary predicates as binary.










% \subsubsection{Binary extensions of unary predicates}
% \label{sec:join}
% % \TODO{citare Neural Logic Machines (nel loro caso usano il verbo expand, ma di fatto fanno la stessa cosa... ma su tensori)}
% Given a unary predicate $P$, we define its binary extensions as two binary predicates $P^x$ and $P^y$
% and impose the constraints: 

%   \begin{align}
%     \begin{array}{c}
% P^x(x,y) \leftrightarrow P(x) \\
%       P^y(x,y) \leftrightarrow P(y)
%     \end{array}
%     \label{eq:binarized-unary-predicates}
%   \end{align}
% Intuitively, $P^x$ and $P^y$ are binary predicates that ignore the second and the first input, respectively. For instance, let $Smoker(x)$ be the unary predicate that is true if person $x$ smokes. The binary atom $Smoker^x(x,y)$ corresponds to the sentence: ``The first element of the pair $(x,y)$ is a smoker''.

% For each binary clause, we can substitute the original unary predicates with their binary extensions. For instance, the clause
% $$c: \lnot Smoker(x) \lor \lnot Friends(x,y) \lor Smoker(y)$$
% is converted to
% $$c': \lnot Smoker^x(x,y) \lor \lnot Friends(x,y) \lor Smoker^y(x,y)$$

% It is easy to prove that the truth value of any grounding of $c'$ is the same as the corresponding grounding of $c$:
% $$\Big( Smoker^x(\alice,\bob) \leftrightarrow Smoker(\alice) \Big) \land \Big(Smoker^y(\alice,\bob) \leftrightarrow Smoker(\bob)\Big) \models c[x/\alice,y/\bob] \leftrightarrow c'[x/\alice,y/\bob]$$
% After this transformation, binary clauses can be seen as unary clauses on the domain of pairs of objects on which we can apply KE$_b$. \

% % Notice that while in $c$ there were both unary and binary predicates, in $c'$ all the predicates are binary. This is true for the original domain $O$, but they can be seen as unary predicates if we consider the domain of pairs in $O \times O$. The new solution for the binary knowledge comes exactly from this new perspective: if we extend matrix $\B$ to contain also the new binary predicates $U_i^x$ and $U_i^y$, then we can apply directly the KE on the resulting matrix using $\clauses_B$. 

% % In the relational database analogy, this approach is equivalent to perform a JOIN query on $\U$ and $\B$ and apply the KE on the resulting matrix:

% % \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% % 	*$\M$* = SELECT *$s^x$*, *$s^y$*, *$U_i^x$*, *$U_i^y$*, *$B_j$* 
% % 	     FROM U AS Ux, U AS Uy, B
% % 	     WHERE Ux.*$i$* = B.*$s^x$* AND Uy.*$i$* = B.*$s^y$*
% % \end{lstlisting}
% % where $U_i^x$ is a shortcut for selecting all the unary predicates in Ux
% % (Ux.$U_i$ AS $U_i^x$).

% \begin{figure}[t]
% 	\centering
% 	\input{tikz/JOIN}
%     \caption{The JOIN query: all the binary predicates (including the binary extensions) are collected in a unique matrix. The red numbers are all referring to the same grounded atom $C(o_0)$.}
%     \label{fig:join}
% \end{figure}


% % \TODO{
% % Mapping function just need to return a matrix $\M$ which has a row for each pair of objects and a column for each binary predicate (including the binary extensions $U_i^x(x,y)$ and $U_i^y(x,y)$).}

% \subsection{Relational Data - \kenn\ architecture}
% \label{sec:groupby}


% To cope with ``binarized'' unary atoms, table $\B$ is extended with additional columns for the predicates $P^x_i$ and $P^y_i$ for every unary predicate $P_i$. In order to satisfy the constraints in \eqref{eq:binarized-unary-predicates} the values of these new attributes are computed by joining $\B$ and $\U$ on the indexes $i$, $s^x$ and $s^y$. We denote with $\M$ the result of this join:
% \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% 	*$\M$* = SELECT *$s^x$*, *$s^y$*, *$U_i^x$*, *$U_i^y$*, *$B_j$* 
% 	     FROM U AS Ux, U AS Uy, B
% 	     WHERE Ux.*$i$* = B.*$s^x$* AND Uy.*$i$* = B.*$s^y$*
% \end{lstlisting}
% where $U_i^x$ is a shortcut for selecting all the unary predicates in Ux
% (Ux.$U_i$ AS $U_i^x$).



% % we use the so called \emph{mapping function}, which maps the graph representation into a single matrix $\M$. 
% {%\color{red}
% The matrix $\M$ defined by the JOIN query is used by KE$_b$ with $\clauses_B$. KE$_b$ returns $\delta \M$, a table of the same shape (and same values for $s^x$ and $s^y$) of $\M$. Such table contains the changes on the initial predictions induced by binary clauses. Figure~\ref{fig:join} shows an example of the application of join and KE$_b$.}


% Finally, the different delta values associated with each grounded atom are aggregated together. This can be achieved by the following three queries:

% \begin{lstlisting}[language=SQL, escapeinside={*}{*}]
% 	*$\delta B$* = SELECT *$\delta B_i$*
% 	     FROM *$\delta M$*
	
% 	*$\delta U_x$* = SELECT SUM(*$\delta U_i^x$*)
% 	      FROM *$\delta M$*
% 	      GROUP BY *$s^x$*

% 	*$\delta U_y$* = SELECT SUM(*$\delta U_i^y$*)
% 	      FROM *$\delta M$*
% 	      GROUP BY *$s^y$*
% \end{lstlisting}

% \noindent Figure~\ref{fig:groupby} shows the second query, which is used to calculate the $\delta U_x$. 

% \begin{figure}[H]
% 	\centering
% 	\input{tikz/GROUP_BY}
% 	\caption{An example of a GROUP BY query: for each unary predicate ($S$ and $C$), the values of their first binary extension ($S^x$ and $C^x$) are summed up based on the index 
% 	% \TODO{Dovrei mettere anche la select e renderla piu chiara???}
% 	}
%     \label{fig:groupby}
% \end{figure}


% \noindent The final preactivations $\U'$ and $\B'$ are
% $$\U' = \U + \delta \U_u + \delta \U_x + \delta \U_y$$
% and
% $$\B' = \B + \delta \B$$



% % the \emph{reverse mapping function} takes in input $\delta \M$ and outputs $\delta \U^b$ and $\delta \B$ which are added to $\U$ and $\B$ to obtain the final predictions.}

% \noindent Figure~\ref{fig:unary_binary} shows a high-level overview of the entire model.

% % In the next chapter, the implementation details will be introduced, with a focus on how to implement the four queries introduced in this chapter as differentiable functions.


% \begin{figure}
% 	\centering
% 	\input{tikz/rel_overview}
% 	\caption{
% 	To obtain $\delta \U_u$, unary clauses $\clauses_U$ are used by KE directly on $\U$. The JOIN query is used to find matrix $\M$. Then, the KE is applied to $\M$ using binary clauses $\clauses_B$. Finally, to obtain $\delta \U_b$ and $\delta \B$ other three queries are used.}
%     \label{fig:unary_binary}
% \end{figure}




% \subsection{Knowledge for inputs/outputs relationships}
% \label{sec:KENN_inputs}
% Until now, we defined \kenn\ as a method that injects logical knowledge which represents relationships between different predictions of a Neural Network. However, it is even possible to provide knowledge which expresses relationships between inputs and outputs values. In other words, if some of the inputs are truth values of some atomic formulas, we can add clauses that contain them, providing in this way information on the relations between inputs and outputs. 

% Figure~\ref{fig:KENN_inputs} introduces this idea: the solution is straightforward, we just need to concatenate the inputs of the base NN with its outputs before applying the KE. The KE will provide an updated version of both inputs ($\bx'$) and outputs ($\by'$). Since we are interested only in the outputs, the last step discards the changed inputs $\bx'$.

% \begin{figure}[H]
% 	\centering
% 	\input{tikz/KENN_inputs}
% 	\caption{KENN used with knowledge on both inputs and predictions: the ``preactivations'' $\bz_x$ of inputs $\bx$ are calculated with the logit function and concatenated to the preactivations of the outputs $\by$. The result can be used by KE to force the satisfaction of the knowledge.}
% 	\label{fig:KENN_inputs}
% \end{figure}

% Notice that, since the KE works with preactivations, the logit function (the inverse of logistic function) must be applied to the inputs before the concatenation. Moreover, the logit is defined in the range $(0,1)$, which means that if the truth values in $\bx$ are zeros and ones, logit can not be applied directly. For this reason, a small number $\epsilon$ is added or subtracted to $\bx$ before applying the logit. Alternatively, $\bz_x$ can be set to a high value when $\bx$ is positive and a very high negative number when it is negative (in our experiments we used 500 and -500).
% %  to keep the values of $\bx$ in the domain of the logit function.

% % \section{Mapping function}
% % \TODO{spostare in implementazione e sistemare}
% %  The mapping function makes use of \emph{gather} function of TensorFlow which slices a given matrix according to an indices vector. In Fig.~\ref{fig:gather} an example of \emph{tf.gather} usage. For more details about \emph{tf.gather} see the official \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation}.

% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/gather_example}
% %     \caption{\emph{tf.gather} behaviour: given a matrix $\U$, it copies in a new matrix the rows of $\U$ based on the provided indices.}
% %     \label{fig:gather}
% % \end{figure}

% % Vectors $s^x$ and $s^y$ contain the indexes of the objects in $\U$ which are referred by matrix $\B$. For instance, in Fig.~\ref{fig:gather} $s^y_0=1$, which means that in the first row of $\B$ the $y$ variable of the binary predicates is substituted by object $\bob$ . Therefore, when \emph{tf.gather} is applied to $\U$ using $s^x$ ($s^y$) it generates a matrix containing the values of $U_i^x$ ($U_i^y$) corresponding to the grounding in $\B$. The mapping function just need to concatenate the resulting matrices with $\B$ to obtain the final matrix $\M$. Fig.~\ref{fig:mapping}~shows the implementation of mapping function.

% % The key point of this strategy is that we can apply the KE on matrix $\M$ using $\clauses_B$. The result $\delta \M$ is a matrix of the same shape of $\M$ which collects all the changes to be applied on atomic formulas due to binary clauses.

% % Now we just need to define the reverse mapping function, which copies $\delta \M$ values into the initial representation: it returns the final changes (generated from $\clauses_B$) that should be applied on unary ($\delta \U^b$) and binary ($\delta \B$) grounded predicates.

% % % to copy the unary predicates in the right spots of final matrix $\M$ (see \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation} for a better description of \emph{tf.gather} function).

% % % In the shown example:
% % % $$
% % % s^x = \ensuremath{\begin{pmatrix}0\\0\\1\\1\\2\\2\end{pmatrix}}
% % % $$

% % % This is telling us that the first two rows of matrix $\B$
% % % % and of the final matrix $M$
% % % are referring to the object in row $0$ of $\U$, while the third and fourth row correspond to row $1$ in $\U$. By applying \emph{tf.gather} to matrix $\U$ and vector $s^x$ we generate a matrix which contains the unary predicates values for the objects referred by $s^x$. The same strategy is applied with $s^y$. Finally we concatenate the two resulting matrices with $\B$. The final matrix $\M$ can be seen as an extension of matrix $\B$ obtained by adding the missing binary predicates (the binary extensions of unary predicates). 



% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/rel_mapping}
% %     \caption{\TODO{usare anche qui l'esempio, specificare almeno una regola logica e mettere dei valori sensati..., aggiungere altra immagine separate per l'applicazione del KE (sempre con lo stesso esempio) in cui si mostra esattamente cosa succede} The architecture of mapping function: it applies \emph{tf.gather} to $\U$ using as indices $s^x$ and $s^y$. The resulting matrices contain $\U$'s rows ordered as specified by the two vectors. Finally, using the concatenation it generates matrix $\M$ which can be provided as input to the KE together with the binary knowledge $\clauses_B$.}
% %     \label{fig:mapping}
% % \end{figure}



% % \section{Reverse mapping function}
% % \label{reverse}
% % \TODO{spostare in implementazione e sistemare}

% % From Fig.~\ref{fig:mapping} we can notice that we have multiple delta values for each grounded unary predicate inside matrix $\delta \M$. For instance, the values of $M_{0,2}$, $M_{2,0}$, $M_{3,0}$ and $M_{5,2}$ are all referring to $U_1(\bob)$ and they come from different grounding of the binary clauses.

% % The reverse mapping function works in reverse of the mapping function. The first step is to split $\delta \M$ in three matrices: $\delta \M^x$ contains the delta values for predicates of the form $U_i^x$, $\delta \M^y$ refers to predicates $U_i^y$ and $\delta \B$ to binary predicates $B_j$. 

% % % \AD{Notice that $\delta \M^x$ does not contain any predicates that refers to variable $y$ (the same is true for $\delta \M^y$ and variable $x$). Therefore, we can see the predicates referred by $\delta \M^x$ as the original unary predicates (instead of using their binary extensions). Indeed, $\delta \M^x$ has a similar structure as $\U$, with the exception that multiple rows refer to the same object.}

% % The proposed changes for binary predicates ($\delta \B$) are already usable. In other words, they can be directly added to matrix $\B$ to obtain final preactivations $\B'$: 
% % $$\B' = \B + \delta \B$$

% % For the unary predicates it is needed an additional step: we have to collect all the changes referring to the same atomic formula, sum them together and put the results in the right position of matrix $\delta \U^b$. This is achieved through the use of \emph{scatter\_nd} function of TensorFlow which works in reverse of \emph{tf.gather}. Indeed, while for \emph{tf.gather} the indices refer to the input matrix, with \emph{tf.scatter\_nd} they refer to the output matrix. Fig.~\ref{fig:scatter} shows an example of \emph{tf.scatter\_nd} usage (see \href{https://www.tensorflow.org/api_docs/python/tf/scatter_nd}{TensorFlow documentation} for more details). Notice that when the indices vector contains multiple indices with the same value, the corresponding rows are summed together before being copied. 

% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/scatter_example}
% %     \caption{\emph{tf.scatter} behaviour: it copies the rows of a matrix in the specified indices. When multiple indices are equivalent it sums the corresponding rows.}
% %     \label{fig:scatter}
% % \end{figure}

% % Using \emph{tf.scatter\_nd} with indices vector $s^x$, \kenn\ can automatically sum up all the contributions of the same atomic formula found in $\delta \M^x$ and put the results in the right position inside a new matrix called $\delta \U^x$. The same strategy is applied for calculating $\delta \U^y$ matrix. Then the two matrices are summed together to obtain $\delta \U^b$:
% % $$\delta \U^b = \delta \U^x + \delta \U^y$$
% % Finally, the preactivations of unary predicates are calculated as:
% % $$\U' = \U + \delta \U^u + \delta \U^b$$

% % The detailed architecture of the reverse mapping function can be seen in Fig.~\ref{fig:reverse_mapping}.


% % \begin{figure}[t]
% % 	\centering
% % 	\input{tikz/rel_reverse_mapping}
% %     \caption{\TODO{Continuare anche qui con l'esempio solito} The architecture of the reverse mapping function: first, it splits $\delta \M$ into three matrices which contain the improvements to apply to predicates $U_i^x$, $U_i^y$ and $B_i$. It then makes use of \emph{tf.scatter\_nd} to add all the values referring to the same atomic formulas and store them in the right position in $\delta \U^x$ and $\delta \U^y$. Finally, the two matrices are added together to obtain $\delta \U^b$.}
% %     \label{fig:reverse_mapping}
% % \end{figure}


% % % \begin{figure*}
% % %     \makebox[\textwidth][c]{
% % %         \includegraphics[scale=0.09]{reverse_mapping.jpg}
% % %     }
% % %     \caption{The reverse mapping function projects the changes proposed by KE (with binary clauses $\clauses_B$) into the original data structure of the underlying graph. It makes use of \emph{tf.scatter\_nd} function, which works in reverse as \emph{tf.gather}: it sums up all the rows in $\delta \U^x$ that refer to the same object in $O$. In other words, it sums rows with the same value in $s^x$. The same is done for $\delta \U^y$ and $s^y$. The final matrices has the same shape as $U'$ and they are summed to it to obtain the final unary predictions $U$.}
% % %     \label{fig:reverse_mapping}
% % % \end{figure*}





% % {


% % % \begin{TODO LIST}{TODO}
% % %     \item Aggiungere spiegazione formale del perche' e' corretto (scatter\_nd calcola la somma su tutti i groundings...)
% % %     \item aggiungere in appendix descrizione di scatter\_nd e gather
% % % \end{TODO LIST}


% % }




% % % \TODO{
% % % Figure~\ref{fig:CE} shows in details the architecture of \kenn's last layer. KE is a function that takes as input the preactivations ${\bz}$ of the base NN and produces the final activations ${\by'}$. In the picture, $\bz$ is visualized as a vector. However, in the general case it is a matrix whose columns represents a predicate and each row an object. In other words, element $z_{ij}$ represents the preactivation of $P_j(o_i)$, where $P_j$ is the $j^{th}$ predicate, and $o_i$ the $i^{th}$ object. This representation restricts the scenarios where we can apply \kenn: it can be used in the context of multi-label classification, but it is not straightforward to use it in the presence of both unary and binary predicates. In Chapter~\ref{ch:srl} we will see how to extend \kenn \ to work with relational data as well.



% % % Internally, for each clause $c \in \clauses$, KE has a sub-module called \emph{Clause Enhancer} (CE), which returns $\delta_c^z$, the adjustments to be applied on preactivations to enforce $c$ satisfaction. Such values are also stored in a matrix of the same shape of $\bz$. In this way it is easy to aggregate all the contributions for different clauses: CEs outputs are combined linearly using \emph{clauses weights} and summed to the initial preactivations.}

% % % Lastly, the final predictions are calculated by applying the logistic function:

% % % \TODO{
% % % \begin{equation}
% % %   \label{eq:ke}
% % %   y'_i = \sigma\Big(z_i + \sum_{c \in \clauses \atop i \in c} 
% % %   \sign_{c,i}\cdot \delta^{w_c}_s(\bsign_c\odot {\bz}_c)_i \Big)
% % % \end{equation}

% % % Cambiare formula (usando la notazione precedente): la predizione di una formula atomica e' la somma tra la predizione iniziale e la somma dei vari delta generati dai CE... (riferirsi a questa formula dopo, nell'implementazione (dove si deve mostrare che effettivamente e' quello che otteniamo usando la matrice z e gather) e nella parte relazionale (in quel caso si deve distinguere tra predicati unari e binari e mostrare che con mapping e reverse mapping otteniamo esattamente quello che vogiamo))}

% % % \noindent where $i\in c$ means that the clause $c$ contains a positive or negative literal corresponding to the preactivations $z_i$, $\bz_c$ are all the preactivations corresponding to the literals in $c$, $\odot$ is the element-wise multiplication, and $\bsign_c$ is a polarity vector of $1$ and $-1$, with $\sign_i=1$ if the $i^{th}$ literal of the clause is positive and $\sign_i=-1$ if it is negative.

 

% % % \chapter{KENN for Statistical Relational Learning}\label{ch:srl}

% % % % \newcommand{\ad}[1]{{\color{blue}#1}}

% % % \begin{TODO LIST}{TODO}
% % %     \item Espandere descrizione:
% % %     \begin{itemize}
% % %         \item Far capire perche la prima versione di \kenn \ non puo essere usata coi dati relazionali (facendo riferimento anche al nuovo capitolo sull'implementazione)
% % %         \item Concantrarsi sul l caso con regole n-arie, e specificare in seguito che nella partica si arriva di solito a arieta 2 o 3 e che ho testato solo con 2 (esempio e immagine con arieta' 2 per semplicita di esposizione)
% % %         \item Usare l'esempio pratico dei documenti (per tutto il capitolo fare riferimento a tale esempio, mostrando come a partire dalle previsioni iniziali e dalle regole logiche si arrivi alle predizioni finali)
% % %         \item Far capire come i vettori di indici sono passati
% % %         \item mettere in chiaro che gli indici possono essere passati dell'utente finale (per esempio, in riferimento all'immagine della rappresentazione, non ci sono self loop nel grafo... questo solo perche il grafo da rappresentare non aveva self loops)
% % %         \item Aggiunta dimostrazione formale del fatto che con mapping e reverse mapping i delta finali sono ancora la somma dei vari delta su tutti i grounding delle regole logiche (dimostrazione divisa in predicati binari e predicati unari) e di conseguenza si soddisfa la formula introdotta nel capitolo teorico su \kenn
% % %         \item [opt] many sorted logic: aggiungendo una tabella per ogni dominio e usando piu volte la mapping function e la reverse su diverse tabelle e' possibile in teoria gestire diversi domini...\\
% % %         In tal caso, per ogni termine di un predicato si definisce il dominio (come in PSL)
% % %     \end{itemize}
% % % \end{TODO LIST}

% % % \begin{TODO LIST}{TODO}
% % %     \item Aggiunta dettagli implementativi
    
% % % \end{TODO LIST}

% % % The first version of \kenn\ has been developed for multilabel classification. \AD{In this chapter we are interested in extending \kenn\ for relational data, where the single matrix representation introduced in Section~\ref{sec:architecture} can not be used.


% % % Such representation is exploited by \kenn\ to minimize the required computational effort: all the operations can be expressed as matrix operations, which are 
% % % Such representation has an advantage: all the Knowledge Enhancer's internal calculations are implemented as matrix operations, which are particularly efficient when working with a GPU. However, the usage of $\bz$ is limiting since it is not possible to represent both unary and binary predicates in such matrix.
% % % and we would like for \kenn\ to consider also binary predicates, which is not possible with the matrix representation we have seen so far.

% % % \AD{
% % % Although the ideas behind \kenn\ could be applied to other types of tasks,the current implementation requires to represent data in a particular format. For this reason, it is not straightforward to use it in different contexts other than multi-label classification.
% % % }

% % % \TODO{
% % % Although the ideas behind \kenn\ could be applied to other types of tasks, the current implementation requires to represent data in a particular format, which is exploited by \kenn\ implementation to minimize the required computational effort. For this reason, \kenn\ can be applied for solving multi-label classification tasks, but it is not straightforward to use it in different contexts. }

% % % More in details, in the architecture introduced in Section~\ref{sec:architecture}, atomic formulas preactivations
% % % % to be modified
% % % are stored as elements of a matrix $\bz$.
% % % %  with columns representing predicates and rows the \TODO{groundings}. 
% % % \AD{Each column of $\bz$ refers to a unary predicate and each row refers to a specific object of the domain. All the atomic formulas in the row are obtained by substituting the free variable of a unary predicate (the one corresponding to the column) with that object.} Such representation is limiting and we would like for \kenn\
% % % % to be more flexible on the data structure used to store atomic formulas' values. We would like 
% % % to consider also binary predicates,\ which is not possible with the matrix representation we have seen so far.
% % % % \TODO{(spostare) each row of $\bz$ refers to a specific object of the domain and all the atomic formulas in the row are obtained by substituting the free variable of a unary predicate with that object.}

% % % We want to extend \kenn\ to work with graphs: instead of focusing only on unary predicates we need to use binary predicates as well. 
% % % The next sections introduces the extension of \kenn\ for relational data, which can be applied on graphs.
% % %  mantaining the good time performances obtained by the usage of the single matrix representation. 
% % % In designing this extension I paid particular attention to maintain the computational efficiency we have obtained in the previous version.}


% % %it would be preferable to keep the good time performances obtained by the usage of the single matrix representation. 


% % % \TODO{
% % % The idea is to develop a mapping function $m$ which can convert a custom representation into the matrix representation used so far. Moreover, we need a reverse mapping function $r$ which converts back the results to the required representation. In this way, we could keep the same implementation of KE.

% % % (reduce the graph problem to the original one...)




% % % % \begin{figure*}
% % % %     \makebox[\textwidth][c]{
% % % %         \includegraphics[scale=0.4]{imgs/m.jpg}
% % % %     }
% % % %     \caption{\kenn\ architecture: (a) for multilabel classification; (b) with structured NN output}
% % % %     \label{fig:mapping}
% % % % \end{figure*}


% % % In Fig.~\ref{fig:mapping}(a) it is shown the original version of \kenn: a neural network (NN) returns preactivations $\bz'$ based on features $\bx$, then \emph{Knowledge Enhancer} (KE) function takes $\bz'$ as input and returns $\delta \bz$, the update to be added to $\bz'$ in order to obtain the final preactivations $\bz$ (which in turn will be feed to the logistic function). Notice that the image is slightly different from the one of the original paper where the sum between $\bz'$ and $\delta \bz$ were performed inside KE together with the application of logistic regression. However, for the sake of this document, this representation is more useful.

% % % In Fig.~\ref{fig:mapping}(b) it is shown a new version of \kenn: here the results of the neural network have a different representation. Before applying KE, we use mapping function $m$ to store NN predictions into a matrix $M$ that can be processed by KE. A reverse mapping function $r$ is used to change the representation of KE outputs $\delta \M$ (changes to be applied to initial predictions) into the original representation and only then $\bz'$ and $\delta \bz$ are combined (notice that we require the addition to be defined for such a representation).


% % % }
% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "paper KENN"
% %%% End:

